Differentiable Transportation Pruning

Deep learning algorithms are increasingly employed at the edge. However, edge devices are resource constrained and thus require efficient deployment of deep neural networks. Pruning methods are a key tool for edge deployment as they can improve storage, compute, memory bandwidth, and energy usage. In this paper we propose a novel accurate pruning technique that allows precise control over the output network size. Our method uses an efficient optimal transportation scheme which we make end-to-end differentiable and which automatically tunes the exploration-exploitation behavior of the algorithm to find accurate sparse sub-networks. We show that our method achieves state-of-the-art performance compared to previous pruning methods on 3 different datasets, using 5 different models, across a wide range of pruning ratios, and with two types of sparsity budgets and pruning granularities.

==> All_Comment.tex <==
\section{All comments}
\label{Com}


\subsection{From Torsten:}

\begin{itemize}
    \item mask dimension is mismatch: $n$ vs $2$
    \item Without defining training loss first
    \item Using simple sum instead of multiplying with a vector (same as Jan's comment)
    \item score initialization, mention filter pruning maybe first
    \item Optimal Brain Surgeon(OBS): second order Taylor's expansion (we cite in related work)
    \item Compare pruned filters L1 with optimal transport filters: what is the overlap? Can we do this given that we retrain the weighs?  (\yq{TODO in exp})
    \item Why does L1 norm goes to zero for pruned weights Optimal transport often used in mixture of experts (maybe because the used Weight decay...need to justify \yq{TODO in exp})
    \item Compare to 2nd order technique (wood fisher for smaller models, MFAC for large transformer models)
\item Iterative magnitude pruning (neural magic) needs lots of hyperparam tuning but shows what we can achieve ( useful for practitioners)   (This will be sure to do after CVPR deadline for a strong baseline)
\end{itemize}

\subsection{From Bert:}

Great paper with great results! What I'm missing is more focus on how and why this method applies so well to filter pruning and how it intuitively outperforms prior work. I think the section describing the method requires significant rewriting: None of the mathematics or method in itself is actually new as far as I can tell. If that is the case, I think you should (1) more concisely and accurately summarize the optimal transport problem and it's relaxation and (2) spend more time on specifiying the concrete parameters of the formulation and how that matches to the pruning problem. That section was not very clear to me. 

On top of that, I think you need a strong introduction that (1) better sketches the need for better optimized and smaller network architectures. (I could help with that if required) (2) that illustrates how current pruning methods are insufficient and (3) how your method theoretically and practically outperforms the prior work.

\begin{itemize}
    \item I'm missing a good introduction that (A) illustrates why pruning is useful in Neural Network Acceleration, (B) discusses what the problems and limitations are of current pruning methods, (C) highlights why your solution is such a great idea and what is novel about it and finally (D) highlights some of your key results. Such an introduction also simplifies the internal review process.
    \item Why don't you also validate your approach on unstructured pruning? Do you outperform other methods there as well? Would be very intersting to see the results. (we think it, as time-consuming, should work well, would validate it after cvpr)
    \item transportation plan is not explained in related work (maybe explain it in intro, \yq{TODO: keep this in mind later}
    \item If I'm not mistaken, you are actually using a hyperparameter in your method. How does this argument hold? (This hyper-parameter is additional to temperature variable, we only use one temperature, others use  temperature hyper + additional sparsity loss hyper.. clarify it) 
    \item Please explain why and how you are using OT in the context of pruning. This is not apparant from this paragraph. At this stage in the paper, it is not clear that you are.
    + THE PREVIOUS SENTENCE IS UN- 094 CLEAR, CAN YOU CLARIFY IT
    (agree, \yq{i will come back to revise it and link it to the pruning}..)
    \item Is this an original contribution of this paper? This should be made very clear. Does it have implications outside of the pruning-field? (yes, it is used in our cited paper later)
    \yq{i will come back to revise it and link it to the pruning}..)
    \item  the training-aware pruning? I revise to "the pruning optimization algorithm using discrete binary mask"
    \item My direct mathematics knowledge is limited, but this section is indeed not clear. You should try to more clearly explain how this optimal transport problem applies so clearly to optimally learning a pruning mask. I would spend less text on the formal mathematics (which is known and prior art), and more time on clearly expressing why it applies.  (Nice i will rewrite it here)
    \item My math is a bit rusty here, but is any of this  relaxation novel?  (This relaxation allows readers to clearly see what optimization objective one should use. The bilevel is famous used in many field, but here we formulated it for pruning learning.)
    \item Exp (1) are  you training the weights and masks together from scratch, or are you starting from a pretrained model.\yq{TODO}
    \item Exp (2) did you reimplement the other methods, or are you taking results from the respective papers
    \yq{TODO}
    \item  Exp (3) are you using exactly the same training schedule as in the references? Or are their subtle differences in the training schedules (from scratch/from pretrained), number of epochs, ...
    \yq{TODO}
    \item Why does accuracy drop from 73+ to 70\%? Why do you start from that baseline for finetuning? (
    the star point shows the test accuracy for the derived pruned architecture by our soft mask before finetuning, the drop is because a large learning rate)
    \item DiffPrune: first time to see (I remove it, this is must because the old version problem)
    \item Did you implement these methods yourself? Or did you get the results from the respective papers? (the
results are taken from the related literatures, I add this line)
\item This statement on explicitly learning importance scores for pruning in an end-to-end fashion should be a part of the framing of this work in the introduction. (\yq{keep in mind})
    \item Overall comments: each section should first give the intuition of the whole idea using English word (\yq{TODO: keep in mind}
\end{itemize}


\subsection{From Jan:}
\begin{itemize}
    \item Toy example: move m1, m2, m3 to corner, and give them coordinates like [0, 0, 1]... (same as Bram's suggestion, done) 
    \item Toy example: Explain all terms like dot.... (will rewrite it later, done)
    \item Give a optimal transportation example independent fig, 2 distribution (done)
    \item Difficult to
understand at this point of the text as these terms have
not been explained (I will avoid the new term before definition)

    
\end{itemize}



\subsection{From Bram:}
\begin{itemize}
    \item geometric median,  Kullback–Leibler divergence... of what?, will revise
    \item How is the loss by hard mask computed in (i)?: ( I compute the hard mask  by the eq.2 and eq.4 with sorting yet the optimal solution, I  explain that)
\end{itemize}

==> Rebuttal/macrosjvg.tex <==
%% janstuff
\usepackage{xcolor}
%\usepackage{todonotes}
\newcommand{\todo}[1]{[{\bf \color{red} TODO: #1}]}
\newcommand{\jvg}[1]{[{\bf \color{blue} JvG: #1}]}
\newcommand{\bv}[1]{[{\bf \color{orange} BV: #1}]}

\newcommand{\changed}[1]{[{\color{red} #1}]}

\newcommand{\removing}[1]{[{\color[rgb]{1.00,0.00,0.50} #1}]}

% \newcommand{\yq}[1]{[{\color[rgb]{1.00,0.00,0.50} #1}]}

\newcommand{\yq}[1]{[{\color{green} Yq: #1}]}
% \graphicspath{{fig/}}

\usepackage{enumitem}

\newcommand{\Eqs}[2]{Eqs.~(\ref{eq:#1}-\ref{eq:#2})}
\newcommand{\Eq}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\eq}[1]{\Eq{#1}}
\newcommand{\Eqn}[1]{Eq~(\ref{eqn:#1})}
\newcommand{\eqn}[1]{\Eqn{#1}}
\newcommand{\fig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\tab}[1]{Table~\ref{tab:#1}}
\newcommand{\tabl}[1]{Table~\ref{table:#1}}
\newcommand{\tabs}[2]{Tables~\ref{tab:#1}-\ref{tab:#2}}
\newcommand{\sect}[1]{Section~\ref{sec:#1}}
\newcommand{\chap}[1]{Chapter~\ref{chap:#1}}
\newcommand{\app}[1]{Appendix~\ref{app:#1}}
\newcommand{\alg}[1]{Algorithm~\ref{alg:#1}}
\newcommand{\foot}[1]{$^{\ref{foot:#1}}$}

\usepackage{amsmath}
% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Sign}{Sign}

\newcommand{\model}{\emph{bi-half}\xspace}
\newcommand{\Model}{\emph{Bi-half}\xspace}

\def\argmax{\operatornamewithlimits{\rm arg\,max}}

\def\argmin{\operatornamewithlimits{\rm arg\,min}}


\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}

\newcommand\eqdef{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily def}}}{=}}}
% \newcommand{\ie}{\textit{i}.\textit{e}.}
% \newcommand{\eg}{\textit{e}.\textit{g}.}
\usepackage{xspace}
% Choose one of the two follwing:
  \newcommand{\latinphrase}[1]{\textit{#1}}  % always italic
% \newcommand{\latinphrase}[1]{\emph{#1}}    % italic in roman text, upshaped in italicized text
% \newcommand{\etal}{\latinphrase{et~al.}\xspace}
% \newcommand{\ie}{\latinphrase{i.e.}\xspace}

%\usepackage[english]{babel}
%\hyphenation{re-identi-fica-tion}


==> discussion.tex <==
\section{Discussion and Future work}
\label{Discussion_futurework}




% Limitation: 

% This work focused on one-shot pruning, \ie the desired pruning rate was at once applied to the network of interest.  Previous work has shown that iterative pruning, which gradually lowers the pruning rate until the target pruning rate has been reached, can improve upon one-shot pruning~\cite{frankle2018lottery}. Iterative pruning can find smaller, yet accurate, models at the cost of extra compute. Optimal Transportation Pruning can be combined with iterative pruning schedules to further reduce the model size and increase the accuracy, something we intend to explore in future work.

% We have applied Optimal Transportation Pruning in the context of filter pruning because it can generally improve storage, compute and memory usage irrespective of the specific hardware being considered. Despite its hardware friendliness however, filter pruning is quite  restrictive as it removes entire filters from the network. Unstructured pruning on the other hand has less constraints and provides more flexibility to reduce the network at higher accuracy. In future work we intend to apply Optimal Transportation Pruning to semi- and unstructured pruning settings.

To compare our method to previous research we employed predefined sparsity ratios for each layer, which limits the search space of sparse models. We therefore expect that our results can be improved upon by relaxing this constraint and allowing different pruning rates for different layers or (similarly) by applying the learned mask across all layers of the network at once instead of individually per layer (\RVC{See the global sparsity analysis on MobileNetV2 above}). Furthermore, our method can be combined with meta pruning techniques that automatically search the best pruning rates for each layer~\cite{liu2019metapruning} (\RVC{See the budget-aware pruning analysis in \ref{flopslatency}}).

%We also only employ our method witha predefined sparsity ratio per layer currently that may limit the search of a smaller sparse model. Clearly, our method can be used to any other methods that find more proper pruning ratios. In future work, we plan to apply our method on the techniques that will automatically distribute sparsity among layers.



% Our soft mask can automatically anneal to the optimal hard mask with a 
% good  temperature initialization. 
%Our method simply initializes the temperature hyper-parameter to  same over all layers,  but  the  initialization of our  temperature hyper-parameter is sensitive to the soft mask size \bv{we did not show this so I leave it out for now}, \ie the filter size per layer. 
%Distributing a same initialized temperature  over all layers may hamper the training and final performance. 
%In the future we will consider applying our method for network-wise pruning instead of layer-wise pruning that allows setting a single sparsity ratio over the  whole network. 
%Our soft mask learning may also further improve the convergence by finding a proper temperature decaying strategy.

The learnable soft masks on which our method relies may also find usage in other contexts, besides pruning, that rely on discrete optimization. For example dynamic neural network~\cite{han2021dynamic}, which dynamically adjust the network architecture based on the observed activity pattern, build on discrete decisions during training and inference. Similarly, mixture of experts models~\cite{yuksel2012twenty} choose the relevant expert out of a discrete set of possibilities. These methods may benefit from similar techniques as those used in Optimal Transport Pruning, and from optimal transport in general.

%In the future, we will also explore the possibility of applying our method on meta pruning~\cite{liu2019metapruning} that searches for the best pruned architecture by exploring different channel configurations which may further improve the performance. In addition, our soft mask learning may also lead benefits and provide insights on other discrete optimization related fields, for example, on dynamic neural networks that always apply a weight mask based on activation maps to dynamically select proper model size for  different tasks and datasets. 
%One other potential future work for improving our soft mask learning is to explore learning dual variables using stochastic gradient descent instead of using block coordinate ascent based Sinkhorn algorithm.
% in the future, we will explore learning dual variables using 
% stochastic gradient descent.
% Binary network, hashin

% of the  searching different 
% the
% number of channels for the sparse model












 
% 1.the proximal step size can not be set equally for all layers, one potential solution could divide the filter numbers into few groups, each group has the same filter.

% 2. We employ pre-specified pruning ratios in this work to keep the core method neat. Exploring layer-wise sensitivity is out of the scope of this work,
% but clearly any method that finds more proper pruning ratios can readily work with our approaches.
% The main consideration is that pruning ratio is broadly believed to reflect
% the redundancy of different layers LeCun et al. (1990); Wen et al. (2016); He et al. (2017), which
% is an inherent characteristic of the model, thus should not be coupled with the subsequent pruning
% algorithms.

% Future work:  decide the per-layer sparsity automatically and optimally.

% searching the optimal channel configuration

==> experiments_backup.tex <==



\section{Experiments}
\label{exp}

% \textbf{Restructured the Exp:}
% \begin{itemize}
%     \item 
% \end{itemize}


\begin{figure*}[t]
\centering
\begin{tabular}{ccc}
     \includegraphics[width=0.43\textwidth]{figure/scores_all/Toghether3maskIter_independencescore1.pdf} &
         \includegraphics[width=0.542\textwidth]{figure/scores_all/imagenet_acc_mask1.pdf}  
         \\  
         \ \ \ \small{(a) 
  On CIFAR-10}  &
  \small{(b) On ImageNet}
    \end{tabular}
    \caption{ 
    Convergence analysis experiments.
   \textit{(a).} 
   Evolution  of the soft masks associated with three filters from
    ResNet-56 trained on CIFAR-10 with $\varepsilon = 1$.   
 Early in training our method explores different filter compositions.  In later training phases the soft masks have converged to hard
masks. For each mask, the soft mask, importance score and L1 norm of the respective filter are correlated. 
% \htor{why do all scores go towards zero (not corr with masks at 1!)}
  \textit{(b).} 
    Experiments with ResNet-50 on ImageNet with $\varepsilon = 0.25$.  
  After training the soft mask has converged to a discrete hard mask solution. 
The L1 norms of the filters are highly correlated with the soft masks. 
% \htor{can we put L1 on a different scale on the right side so one can see the corr clearer?}.
Bottom: Validation accuracy during training with differential transportation pruning and during finetuning. 
The star point shows the test accuracy for the derived pruned architecture by our soft mask before finetuning. 
% \htor{maybe annotate the regions in the plot?} 
    }
 \label{fig:soft_evo}
\end{figure*}





\begin{table*}[t]
\centering
\small
\parbox{.67\linewidth}{{
\centering
\caption{Various pruning ratios with ResNet-56/VGG-19 on CIFAR-10/CIFAR-100:  
	Accuracy comparison with  GReg-1 \cite{wang2021neural} and $L_1$+one-shot~\cite{li2017pruning}.
  Baseline accuracy for ResNet-56 is 93.36\% and for VGG-19 is 74.02\%.
  Each experiment is repeated 3 times with random initialization, mean and std accuracies are reported.
    }
	\renewcommand{\arraystretch}{1.6}
	\resizebox{1\linewidth}{!}{
	 \setlength{\tabcolsep}{0.005mm}{
	   	\begin{tabular}{llccccc}
    	\toprule
		\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}ResNet-56\\(CIFAR-10)\end{tabular}} & 	 Pruning ratio (\%) & 50  & 70 &  90  & 92.5 & 95 \\
   		 & Sparsity (\%) / Speedup & 49.82/1.99$\times$  & 70.57/3.59$\times$  &  90.39/11.41$\times$   & 93.43/14.76$\times$  & 95.19/19.31$\times$  \\
      % \midrule	
      \cline{2-7}
		 & $L_1$+one-shot (Acc.\%)~\cite{li2017pruning} & 92.97$\pm$0.15  & 91.88$\pm$0.09 &  87.34$\pm$0.21 &  87.31$\pm$0.28 &  82.79$\pm$0.22 \\
	 &	 GReg-1 (Acc. \%)~\cite{wang2021neural}  & 93.06$\pm$0.09  & 92.23$\pm$0.21 &  89.49$\pm$0.23 &  \textbf{88.39$\pm$0.15} &  85.97$\pm$0.16 \\ 		
	 &	  Ours (Acc. \%) & \textbf{93.46$\pm$0.18}
    &  \textbf{92.46$\pm$0.10}
    &   \textbf{89.84$\pm$0.14}
    &   {88.03$\pm$0.33}
    & \textbf{86.18$\pm$0.06} \\ 		
	   % \bottomrule
     \midrule	
    \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}VGG-19\\(CIFAR-100)\end{tabular}}  &	Pruning ratio (\%) & 50  & 60 &  70  & 80 & 90 \\
    &		 Sparsity (\%) / Speedup & 74.87/3.60$\times$  & 84.00/5.41$\times$  &  90.98/8.84$\times$   & 95.95/17.30$\times$  & 98.96/44.22$\times$  \\
      % \midrule
       \cline{2-7}
	 &	 $L_1$+one-shot (Acc.\%)~\cite{li2017pruning} & 71.49$\pm$0.14  & 70.27$\pm$0.12 &  66.05$\pm$0.04 &  61.59$\pm$0.03 &  51.36$\pm$0.11 \\
	 &	 GReg-1 (Acc.\%)~\cite{wang2021neural}  & 71.50$\pm$0.12  & 70.33$\pm$0.12 &  67.35$\pm$0.15 &  63.55$\pm$0.29 &  57.09$\pm$0.03 \\ 		
 &		 Ours (Acc. \%) & \textbf{71.56$\pm$0.19}
    & \textbf{70.41$\pm$0.06}
    &   \textbf{67.74$\pm$0.13}
    &   \textbf{63.98$\pm$0.25}
    &   \textbf{57.21$\pm$0.09}
    \\	
	   \bottomrule
	\end{tabular}
	}}
	\label{tab:resnet56_vgg_cifar}
}}
\hfill
\begin{minipage}{.31\linewidth}
\centering
\caption{ \RVC{MobileNetV2 on CIFAR-10/100 with global sparsity ratio over network. }}
% \vspace{-0.1in}
\parbox{1\linewidth}{{
\centering
% \vspace{-0.1in}
	    \renewcommand{\arraystretch}{1}
		\setlength{\tabcolsep}{1.5mm}{
	\resizebox{1\linewidth}{!}{
		\begin{tabular}[c]{lc|ccccccc}%{C{4cm}|C{2cm} C{2cm}}
			\toprule
			\multirow{2}{*}{Method} &  \multirow{2}{*}{Sparsity (\%)} & \multicolumn{2}{c}{Acc.} \\
			& & CIFAR-10 & CIFAR-100   \\
			\midrule
   	Unpruned  & 0 &  93.70 & 72.80
   \\
			\midrule

			% ChipNet  &\multirow{2}{*}{80}& 92.23  & 72.25     \\
			% Ours && 92.33 & 72.61    \\
   % \midrule			
   % ChipNet  &\multirow{2}{*}{60}& 92.24 &   70.62    \\
			% Ours && 92.54 &    71.49      \\
   % \midrule
   			ChipNet~\cite{tiwari2021chipnet}  &\multirow{2}{*}{60}& 91.83 & 66.61    \\
			Ours && \textbf{91.93} &  \textbf{70.45}     \\
   \midrule
   			ChipNet~\cite{tiwari2021chipnet}  &\multirow{2}{*}{80}& 90.41   & 52.96    \\
			Ours &&  \textbf{91.49} &  \textbf{68.90}     \\
			\bottomrule
		\end{tabular}
	} \label{tab:gloabalsparsity}	
}	
}}
\parbox{1\linewidth}{{
\vspace{0.05in}
\centering
 	\caption{\RVC{
	Unstructured pruning on ImageNet for ResNet-50.
    }}
    % \vspace{-0.1in}
	    \renewcommand{\arraystretch}{1}
		\setlength{\tabcolsep}{.5mm}{
	    \resizebox{1\linewidth}{!}{
		\begin{tabular}[c]{lcccccccccc}
		\toprule			
        \multirow{2}*{Method}  &  
        % \multirow{2}*{Backbone} & 
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Baseline\\Acc.(\%)\end{tabular}}
        % \multirow{1}*{Baseline Top-1 Acc (\%)} 
        &   
                \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pruned\\Acc.(\%)\end{tabular}}
        % Pruned Top-1 Acc (\%) 
        & 
                        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Droped\\ Acc.(\%)\end{tabular}}
        % {Top-1 Acc drop (\%) }
        & 
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Sparsity\\ (\%)\end{tabular}}
   % \multirow{2}{*}{} 
        \\
        \\\midrule
   GSM~\cite{ding2019global} & 
   % \multirow{7}*{ResNet-50} &
   75.72  &  74.30&   1.42 &  80.00 \\ % 
      Sparse VD~\cite{molchanov2017variational} 
      % &
      & 76.69 &    75.28 &  1.41 & 80.00   \\	
DPF~\cite{lin2020dynamic} &  
75.95 &    74.55 &  1.40 &  82.60  \\	
% 		& Real2Binary & 1/1 &  60.9 & 83.0  \\
WoodFisher~\cite{singh2020woodfisher} & 
% & 
75.98 &   75.20 &  0.78 &  82.70  \\	
% 		& Real2Binary & 1/1 &  60.9 & 83.0  \\
       GReg-1~\cite{wang2021neural} 
       % & 
       &  76.13 &  75.45 &  0.68 & 82.70           \\	
              GReg-2~\cite{wang2021neural} 
              % &
              &  76.13  &    75.27 &  0.86 & 82.70        \\	
              Ours 
              % &
              &   76.13  & \textbf{75.50}  &  \textbf{0.63} & 82.70   \\	       
        \bottomrule
		\end{tabular}
  }
  }
\label{tab:imagnet_unstru}
}}
\end{minipage}
\end{table*}




% \begin{itemize}
%     \item Type 1: 
% % sub-network vs iteration in heatmap (x-axis: iteration; y-axis: mask values) 
% \item soft-mask, L2 norm / independence score vs. iteration   \yq{Done}
% \item \yq{Done}
% Show the final-trained masks over one layer on imagenet and test acc curve 
% % show why this sub-network is best: sample several subnetwork and give same weights value
% % \item 
% % show the kept weight values is important: using same arch + different weight values
% \item Type 2: 
% how ours perform with different T (temperature)
% \item Different order: 1st order and 2nd order
% \item 
% integrate with others such as Reg-based methods (different pruning rate): Reg / Ours / Ours + Reg ..
% \item  independence score or L2 norm score of filters?
% \item STE vs ours
% % exam six different importance-based criterions?
% \item Type 3: \yq{Done}
% ResNet-56 + CIFAR-10
% VGG19 + CIFAR-100
% ResNet-34 / ResNet-50 + ImageNet
% \end{itemize}


% \textbf{Datasets and training details.}
% We conduct the experiments on  CIFAR-10, CIFAR-100 and ImageNet datasets using ResNet-56, VGG19
% Our experiments for CIFAR-10 and CIFAR-100 datasets are conducted on ResNet-56 and VGG19 respectively. 
% We validate our proposed method on different models and datasets 
% by applying filter pruning to the weights of a network. 
\RVC{
We validate our proposed method mainly on filter pruning  using different models and datasets, and then extend to unstructured pruning.}
Filter pruning is a form of structured pruning that removes entire filters from the layers of a network, thereby compressing the network, and potentially accelerating the network by reducing the number of FLOPs needed to execute it.

\noindent \textbf{Datasets and networks.}
We first conduct our experiments on CIFAR-10 with ResNet-56 and on CIFAR-100 with VGG-19. 
Following~\cite{wang2021neural}, for the CIFAR datasets we train our baseline models with accuracy comparable to those in the original papers. 
% \bv{TODO:REPORT BASELINE ACCURACIES IN TABLE 1}. %\htor{also double-check paperswithcode for updated baselines}
We then evaluate our method on the large-scale ImageNet dataset with ResNet-34 and ResNet-50. Following~\cite{wang2021neural}, we use the PyTorch~\cite{paszke2019pytorch} pretrained models as our baseline models. 
\RVC{
We also apply our method to prune lightweight architecture MobileNetV2. 
}

% \begin{table*}[t]
% 	\centering
%  	\caption{Various pruning ratios with ResNet-56/VGG-19 on CIFAR-10/CIFAR-100:  
% 	Accuracy comparison with  GReg-1 \cite{wang2021neural} and $L_1$+one-shot~\cite{li2017pruning}.
%   Baseline accuracy for ResNet-56 is 93.36\% and for VGG-19 is 74.02\%.
%   Each experiment is repeated 3 times with random initialization, mean and std accuracies are reported.
%     }
% 	\renewcommand{\arraystretch}{1.6}
% 	\resizebox{0.95\linewidth}{!}{
% 	 \setlength{\tabcolsep}{3.5mm}{
% 	   	\begin{tabular}{llccccc}
%     	\toprule
% 		\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}ResNet-56\\(CIFAR-10)\end{tabular}} & 	 Pruning ratio (\%) & 50  & 70 &  90  & 92.5 & 95 \\
%    		 & Sparsity (\%) / Speedup & 49.82/1.99$\times$  & 70.57/3.59$\times$  &  90.39/11.41$\times$   & 93.43/14.76$\times$  & 95.19/19.31$\times$  \\
%       % \midrule	
%       \cline{2-7}
% 		 & $L_1$+one-shot (Acc. \%)~\cite{li2017pruning} & 92.97$\pm$0.15  & 91.88$\pm$0.09 &  87.34$\pm$0.21 &  87.31$\pm$0.28 &  82.79$\pm$0.22 \\
% 	 &	 GReg-1 (Acc. \%)~\cite{wang2021neural}  & 93.06$\pm$0.09  & 92.23$\pm$0.21 &  89.49$\pm$0.23 &  \textbf{88.39$\pm$0.15} &  85.97$\pm$0.16 \\ 		
% 	 &	  Ours (Acc. \%) & \textbf{93.46$\pm$0.18}
%     &  \textbf{92.46$\pm$0.10}
%     &   \textbf{89.84$\pm$0.14}
%     &   {88.03$\pm$0.33}
%     & \textbf{86.18$\pm$0.06} \\ 		
% 	   % \bottomrule
%      \midrule	
%     \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}VGG-19\\(CIFAR-100)\end{tabular}}  &	Pruning ratio (\%) & 50  & 60 &  70  & 80 & 90 \\
%     &		 Sparsity (\%) / Speedup & 74.87/3.60$\times$  & 84.00/5.41$\times$  &  90.98/8.84$\times$   & 95.95/17.30$\times$  & 98.96/44.22$\times$  \\
%       % \midrule
%        \cline{2-7}
% 	 &	 $L_1$+one-shot (Acc. \%)~\cite{li2017pruning} & 71.49$\pm$0.14  & 70.27$\pm$0.12 &  66.05$\pm$0.04 &  61.59$\pm$0.03 &  51.36$\pm$0.11 \\
% 	 &	 GReg-1 (Acc. \%)~\cite{wang2021neural}  & 71.50$\pm$0.12  & 70.33$\pm$0.12 &  67.35$\pm$0.15 &  63.55$\pm$0.29 &  57.09$\pm$0.03 \\ 		
%  &		 Ours (Acc. \%) & \textbf{71.56$\pm$0.19}
%     & \textbf{70.41$\pm$0.06}
%     &   \textbf{67.74$\pm$0.13}
%     &   \textbf{63.98$\pm$0.25}
%     &   \textbf{57.21$\pm$0.09}
%     \\	
% 	   \bottomrule
% 	\end{tabular}
% 	}}
% 	\label{tab:resnet56_vgg_cifar}
% \end{table*}

% \RVC{
% \begin{table}[t]
% 	\centering
%  	\caption{
% 	Compression comparison on ImageNet with ResNet-50.
%     }
% 	    \renewcommand{\arraystretch}{1.1}
% 		\setlength{\tabcolsep}{1.4mm}{
% 	    \resizebox{1\linewidth}{!}{
% 		\begin{tabular}[c]{lccccclccccc}
% 		\toprule			
%         \multirow{2}*{Method}  &  
%         \multirow{2}*{Backbone} & 
%         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Baseline\\Acc (\%)\end{tabular}}
%         % \multirow{1}*{Baseline Top-1 Acc (\%)} 
%         &   
%                 \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pruned\\Acc (\%)\end{tabular}}
%         % Pruned Top-1 Acc (\%) 
%         & 
%                         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Acc\\Drop (\%)\end{tabular}}
%         % {Top-1 Acc drop (\%) }
%         & 
%     \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Sparsity\\ (\%)\end{tabular}}
%    % \multirow{2}{*}{} 
%         \\
%         \\\midrule
%    GSM~\cite{ding2019global} &  \multirow{7}*{ResNet-50} &  75.72  &  74.30&   1.42 &  80.00 \\ % 
%       Variational Dropout~\cite{molchanov2017variational} &  & 76.69 &    75.28 &  1.41 & 80.00   \\	
% DPF~\cite{lin2020dynamic} &  &  75.95 &    74.55 &  1.40 &  82.60  \\	
% % 		& Real2Binary & 1/1 &  60.9 & 83.0  \\
% WoodFisher~\cite{singh2020woodfisher} &  &  75.98 &   75.20 &  0.78 &  82.70  \\	
% % 		& Real2Binary & 1/1 &  60.9 & 83.0  \\
%        GReg-1~\cite{wang2021neural} & &  76.13 &  75.45 &  0.68 & 82.70           \\	
%               GReg-2~\cite{wang2021neural} & &  76.13  &    75.27 &  0.86 & 82.70        \\	
%               Ours & &   76.13  & \textbf{75.50}  &  \textbf{0.63} & 82.70   \\	       
%         \bottomrule
% 		\end{tabular}
%   }
%   }
% \label{tab:imagnet_unstru}
% \end{table}
% }











\noindent \textbf{Training settings.}
The importance scores corresponding to each layer's filters are initialized to the L2-norm of the respective pretrained filter weights. For fair comparisons, we adopt the same pruning rate schedules as~\cite{wang2021neural}.
% We will apply absute valu
% we will train one mask value for each filter by initializing one importance score.
Also following~\cite{wang2021neural}, for each pruning schedule we denote the model speedup as the pruning-induced reduction in the number of floating point operations (FLOPs) relative to the original model.
The whole training procedure consists of two stages: optimal transportation pruning and post-pruning finetuning. 

Our main focus is on how to train the soft masks in  first stage. 
An important hyperparameter in this respect is  the regularization constant $\varepsilon$.
For ResNet-56 and MobileNetV2, we use $\varepsilon = 1$,  for all other networks we set  $\varepsilon = 0.25$. 
 The model variables and importance scores are  trained with standard Stochastic Gradient Descent (SGD) with a momentum of $0.9$. For CIFAR datasets, a weight decay of $5\times 10^{-4}$ and a batch size of $256$ are used. 
On ImageNet we use a weight decay of $10^{-4}$ and train on 4 Tesla V100 GPUs with a batch size of $64$ per GPU. 
In all experiments except for MobileNetV2 that follows the training settings of~\cite{tiwari2021chipnet}, the initial learning rate is set as $0.1$ and  a cosine learning rate decay is applied. 
In finetuning stage, we employed the same training settings as~\cite{wang2021neural}. 



% \begin{figure}[t]
% \centering
% \begin{tabular}{ccc}
%     \includegraphics[width=0.47\textwidth]{figure/scores_all/Toghether3maskIter_independencescore1.pdf} 
%     % \includegraphics[width=0.295\textwidth]{iclr2023/figure/soft_mask_visual/figure_index48_epoch5.pdf} &
% %         \includegraphics[width=0.32\textwidth]{iclr2023/figure/scores_all/Iter_independencescore.pdf} 
% % \includegraphics[width=0.33\textwidth]{iclr2023/figure/scores_all/Iter_L2norm.pdf}
%     \end{tabular}
%     \caption{ 
%  % As training, our soft mask converges to the original optimal sparse solution.
%  % At starting, all filters have similar importance yet L2 norm, then the importance of pruned filters gradually decreased to zero thus we can safely prune them. 
%     }
%  \label{fig:soft_evo}
% \end{figure}




% \begin{figure*}[t]
% \centering
% \begin{tabular}{ccc}
%     \includegraphics[width=0.57\textwidth]{figure/scores_all/Toghether3maskIter_independencescore1.pdf} 
%         \includegraphics[width=0.27\textwidth]{figure/scores_all/ToghetherIter_independencescore.pdf} 
%     % \includegraphics[width=0.295\textwidth]{iclr2023/figure/soft_mask_visual/figure_index48_epoch5.pdf} &
% %         \includegraphics[width=0.32\textwidth]{iclr2023/figure/scores_all/Iter_independencescore.pdf} 
% % \includegraphics[width=0.33\textwidth]{iclr2023/figure/scores_all/Iter_L2norm.pdf}
%     \end{tabular}
%     \caption{ Experiments on ResNet-56 network with Cifar10 with $\varepsilon = 1$.  
%  % During training our soft mask converges to a discrete hard mask solution. 
%  In early training phases, our method performs exploitation-exploration to search the architecture, and  in later training phases the soft masks have converged to hard
% masks, which highly correlate with the L2 norms of the filters. 
%  % As training, our soft mask converges to the original optimal sparse solution.
%  % At starting, all filters have similar importance yet L2 norm, then the importance of pruned filters gradually decreased to zero thus we can safely prune them. 
%     }
%  \label{fig:soft_evo}
% \end{figure*}




\subsection{Convergence Analysis}
In this section we  demonstrate that during training our soft masks converge to discrete masks. 
For this purpose we conduct experiments with ResNet-56 on CIFAR-10 and \yq{with ResNet-50 on ImageNet. TODO}



% \noindent \textbf{Convergence analysis on CIFAR-10.}
\noindent \textbf{How are soft masks converged on CIFAR-10?}
In \fig{soft_evo}(a), we trained ResNet-56 on  CIFAR-10 with a regularization hyperparameter $\varepsilon = 1$ and a  pruning rate  of 0.5, and visualize the evolution during training of the soft mask, importance score and L1 norm values for three filters. 
Early in training, all filters have similar L1 norms and soft masks. Subsequently, however, the algorithm starts to explore different filter compositions:
The soft mask of filter1 first converges to one, then fluctuates between zero and one, after which it moves back towards one, its final value. The soft masks corresponding to filter2 and filter3 display similar exploratory behavior.  
In later training phases, the soft masks converge to hard masks ($\approx$0 or $\approx$1), and the L1 norm of filters with mask values near zero have gradually decreased to zero, a result of the weight decay term in the loss. Since the mask encodes the neurons' connection information, one could interpret the exploration-exploitation process as performing architecture search. 
% Additional results are presented in  \ref{Additional_ex}.
\subsection{Accuracy vs. number of Sinkhorn steps}
To improve the computational efficiency of our method, we propose an optimal transportation algorithm that requires only a single Sinkhorn iteration to converge. To verify that a single Sinkhorn iteration indeed suffices, we performed experiments on CIFAR-10 with ResNet-56 using a single A10 GPU. In \fig{sinkhorn_iterations} we plot the accuracy and training time as a function of the number of innner Sinkhorn steps. A larger number of Sinkhorn steps significantly increases training time without markedly affecting accuracy. Thus a single Sinkhorn iteration suffices.

\RVC{We measure the wall-clock time for a ResNet-50 on a single A100 GPU for 300 iterations using a batch size of 64 with or without training a pruning mask.
%, the average wall-clock time per iteration is 2.44/2.42 second/iteration. 
The training overhead increases by $\sim$0.5\%, which is generally negligible.}

%\noindent \textbf{Convergence analysis on ImageNet.}
%We trained ResNet-50 on ImageNet with the pruning setting corresponding to 3.06× speedup~\cite{wang2021neural}. \bv{TODO: GIVE EXACT PRUNING SCHEDULE PER SPEEDUP IN APPENDIX}
%In the top row of \fig{soft_evo}(b), we visualize the soft mask and L1 norm of 256 filters from layer 24 of the trained model. Note how all soft masks have converged to hard masks  and   that the L1 norms of the filters are  highly correlated with their corresponding mask values.
%In the bottom row of \fig{soft_evo}(b), we plot the validation accuracy of ResNet-50 during training.
%We first use our method to prune the model for 90 epochs and finetune the pruned model for another 90 epochs. 
%During the first stage, our method searches for the best architecture and reduces the importance of the pruned filters. After 90 epochs we can safely prune the filters without a large impact on the accuracy, in the star point we  test the accuracy for the derived sparse model before finetuning, after which finetuning  helps  to further improve the accuracy.
%At the beginning of finetuning we observe a small accuracy drop since we use a larger learning rate at start.
% \htor{90 epochs seems like a lot in ImageNet - should compare to IMP and others (i.e., how much computation they used in comparison)}
% Pruning the filters with our soft mask 

 

\textbf{\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figure/errobar_sinkhornsteps.pdf}
    \caption{Training cost as a function of the number of inner Sinkhorn steps on CIFAR-10 with ResNet-56 using a single GPU. Each experiment is repeated 3 times with random initialization.
    % we use Pytorch automatic differentiation  to calculate the gradients of Sinkhorn. we
    The training cost for a Sinkhorn step is measured in GPU-hours. 
    % \htor{very nice ablation! Hours/GPU is a really weird cost metric? Why not GPU-hours, or just "compute hours"? \yq{Nice, revise it}
    % }
    Increasing the number of Sinkhorn steps, significantly increases the training cost, but hardly affects the accuracy. 
    A single Sinkhorn step is sufficient for our method.
    % \htor{but accuracy does not improve significantly?\yq{Yes, It did not improve performance, we show here that 1inner step for our soft mask is good }
    % }
    }
    \label{fig:sinkhorn_iterations}
\end{figure} }





% \begin{wrapfigure}{r}{0.27\textwidth}
%     \centering
% \includegraphics[width=0.27\textwidth]{figure/errobar_sinkhornsteps.pdf}
%   \caption{Training cost as a function of the number of inner Sinkhorn steps on CIFAR-10 with ResNet-56 using a single A10 GPU. Each experiment is repeated 3 times with random initialization.
%     % we use Pytorch automatic differentiation  to calculate the gradients of Sinkhorn. we
%     The training cost for a Sinkhorn step is measured in GPU-hours. 
%     % \htor{very nice ablation! Hours/GPU is a really weird cost metric? Why not GPU-hours, or just "compute hours"? \yq{Nice, revise it}
%     % }
%     Increasing the number of Sinkhorn steps, significantly increases the training cost, but hardly affects the accuracy. 
%     A single Sinkhorn step is sufficient for our method.
%     % \htor{but accuracy does not improve significantly?\yq{Yes, It did not improve performance, we show here that 1inner step for our soft mask is good }
%     % }
%     }
% \label{fig:sinkhorn_iterations}
% \end{wrapfigure}



\subsection{Results for ResNet-56/VGG-19 on CIFAR}


%\noindent \textbf{Results across different pruning ratios.}
% \noindent \textbf{ResNet-56/Vgg19 on Cifar.} 
We first explore the effect of applying different pruning schedules on the accuracy of ResNet-56 on CIFAR-10 and VGG-19 on CIFAR-100.
We compare our method to two other pruning methods: L1-norm based one-shot pruning~\cite{li2017pruning} and growing regularization "GReg-1"~\cite{wang2021neural} where the results are taken from the  literature~\cite{wang2021neural}.
We use a simple uniform pruning ratio
scheme, where the pruning ratio is identical across all pruned layers. Following common practice~\cite{gale2019state}, we do not prune the first layer, and for ResNet-56 we only prune the first layer in a residual block (as a result of the restriction imposed by the residual addition) ~\cite{wang2021neural, li2017pruning}. 
We explore a broad range of pruning ratios, covering Speedups between
 $2\times$ and $44\times$.
For fair comparisons, the finetuning scheme (e.g., learning rate schedule, number of epochs, etc.) is identical across all methods.

The results are presented in \tab{resnet56_vgg_cifar}. Note that all pruning methods result in exactly the same pruned weights. Therefore the different observed accuracies between methods result from \emph{how} the weights are pruned.
Our proposed method first performs exploration followed by exploitation. In doing so, our method searches for  best architecture while gradually removing the effect of pruned filters on the network output. Our method 
outperforms L1+one-shot in all examined conditions and GReg-1 for all conditions except one.



% \noindent \textbf{Varying regularization hyperparameter.}
% The regularization term $\varepsilon$ is an important hyperparameter in our experiments. We  explored the sensitivity of our method to this hyperparameter by training Resnet56 on CIFAR10 with a range of different $\varepsilon$. 
% In \tab{temp_diff}, we present the performance of different $\varepsilon$ by training the  Resnet56 network on Cifar10 with  a pruning rate of 0.5. 
% We find that setting a proper $\varepsilon$ is important for achieving better accuracy performance. 
% In the \ref{Additional_ex}, we further visualize the  evolutionary path of soft mask for different hyperparameter $\varepsilon$.




% \begin{figure}[t]
% \centering
% \begin{tabular}{ccc}
%     % \includegraphics[width=0.45\textwidth]{figure/scores_all/imagent_softmask_i21.pdf} \\
% %         \includegraphics[width=0.48\textwidth]{figure/scores_all/imagent_softmask_i1.pdf}      &
% % % \includegraphics[width=0.44\textwidth]{figure/scores_all/imagent_softmask_i11.pdf} \\
%         \includegraphics[width=0.45\textwidth]{figure/scores_all/dependent_1order_acc.pdf}  \\
% %         
%     \end{tabular}
%     \caption{ Comparison between  
%     }
%  \label{fig:dep_1order}
% \end{figure}
% \noindent \textbf{Comparing with STE.}
% \yq{TODO}

% \begin{table}[t]
% 	\centering
%    	\caption{Varying regularization hyperparameter. We compare 5 different $\varepsilon$ by training Resnet56 on CIFAR10 with a pruning rate of 0.9.   Setting a proper $\varepsilon$ is important.
%     }
% 	\renewcommand{\arraystretch}{1.2}
% 	\resizebox{0.99\linewidth}{!}{
% 	 \setlength{\tabcolsep}{11mm}{
% 	   	\begin{tabular}{lcccc}
%     	\toprule
% 		 \multirow{1}{*}{\begin{tabular}[l]{@{}l@{}}Regularization\end{tabular}}   &  \multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}Accuracy (\%)\end{tabular}}  
%    \\
%       \midrule		
% 		 $\varepsilon = 100$  

%    & 87.29  \\
%    $\varepsilon = 10$   & 88.99  \\
%    $\varepsilon = 1$    &\textbf{89.75} \\
%    $\varepsilon = 0.1$   &88.88  \\
%    $\varepsilon = 0.01$  &88.78   \\
% 	   \bottomrule
% 	\end{tabular}
% 	}}
% 	\label{tab:temp_diff}
% \end{table}


% \yq{TODO: with different epsilon to see that if the single step is enough for the training.}


% \noindent \textbf{Independent score \textit{vs} dependent score.}
% Our method employs the importance scores $\mathbf{s}$, which is a set of parameters that is independent of the model weights $\mathbf{w}$. 
% This contrasts to previous methods in which the L1 norm of the filter weights were used as importance scores for pruning. The L1 norm based importance scores are therefore dependent scores. 
% In \fig{dep_1order} we compare between our independent score based method (orange line)  and the L1-norm/dependent score based method (blue line) for five different pruning ratios.
% When the
% pruning ratio is relatively small, the difference between both methods is moderate.  
% With increasing pruning ratio, however, the benefit of our independent score based method becomes increasinlgy obvious. 
% This suggests us to use a set of separate parameters as importance scores for learning soft mask.



% \noindent \textbf{1st order 
% \textit{vs} 2nd order approximation.} TODO:
% In  \fig{dep_1order}, orange line and green line...
% % \noindent \textbf{Combining with others}

% \noindent \textbf{Comparing with STE.} TODO



\begin{table}[t]
	\centering
 	\caption{
	{Acceleration comparison for structured filter pruning on ImageNet}. 
 % \jvg{Table is very large. What is the added value of comparing to more than the top 3 per backbone? I would keep only 3 per backbone. } \jvg{If space is a concern; remove the "venue", "drop perc"} \jvg{why is speedup nog bold? Perhaps better to not use bold numbers at all? (ie: also not for accuracy; as the differences are so small) } \jvg{Note: Over emphasizing minor improvements (bold numbers/improved perc.) is annoying for reviewers} 
 Speedup reflects the reduction on FLOPs. 
 % ResNet-34: 3.66 GFLOPs, ResNet-50: 4.09 GFLOPs.
    }
	    \renewcommand{\arraystretch}{1.1}
		\setlength{\tabcolsep}{1.4mm}{
	    \resizebox{1\linewidth}{!}{
		\begin{tabular}[c]{lccccclccccc}
		\toprule			
        \multirow{2}*{Method}  &  
        \multirow{2}*{Backbone} & 
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Baseline\\Acc (\%)\end{tabular}}
        % \multirow{1}*{Baseline Top-1 Acc (\%)} 
        &   
                \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pruned\\Acc (\%)\end{tabular}}
        % Pruned Top-1 Acc (\%) 
        & 
                        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Acc\\Drop (\%)\end{tabular}}
        % {Top-1 Acc drop (\%) }
        & 
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Speed\\ Up\end{tabular}}
   % \multirow{2}{*}{} 
        \\
        \\\midrule
   L1 (pruned-B)  ~\cite{li2017pruning} &  \multirow{5}*{ResNet-34} & 73.23  &  72.17&   1.06 &  1.32$\times$  \\ % 
      Taylor-FO~\cite{molchanov2019importance} &  & 73.31 &   72.83 &  0.48 & 1.29$\times$   \\	
% 		& Real2Binary & 1/1 &  60.9 & 83.0  \\
       GReg-1~\cite{wang2021neural} & & 73.31 &   73.54 &  -0.23 & 1.32$\times$            \\	
              GReg-2~\cite{wang2021neural} & &  73.31  &   73.61 &  -0.30 & 1.32$\times$           \\	
              Ours & &  73.31  & \textbf{74.28}  &  \textbf{-0.97} & 1.32$\times$   \\	       \midrule	
              % IncReg~\cite{wang2019structured} &  \multirow{15}*{ResNet-50} & 75.60  &  72.47 &   3.13 &  2.00$\times$  \\ 
              % \cmidrule(l){2-5}
    	 SFP~\cite{he2018soft} & \multirow{13}*{ResNet-50}
      & 76.15 &   74.61 &  1.54 &  1.72$\times$     \\	
	 HRank~\cite{lin2020hrank}&    &    76.15 &  74.98 &  1.17 & 1.78$\times$  \\ 	
		 % Taylor-FO \cite{molchanov2019importance} &  & 76.18 &  74.50 &1.68 &   1.82$\times$  \\
		Factorized~\cite{li2019compressing}&  & 76.15 & 74.55 & 1.60 & {2.33$\times$}  \\
				 DCP~\cite{zhuang2018discrimination}&  &  76.01 &  74.95 &  1.06   & 2.25$\times$   \\
		 CCP-AC~\cite{peng2019collaborative} &  &  76.15 &   75.32 & 0.83 & 2.18$\times$  \\
   SRR~\cite{wang2021convolutional}
   &  & 76.13 &  75.11 &  1.02 & 2.27$\times$   \\	         AutoPruner~\cite{luo2020autopruner} & & 76.15 &  74.76 &  1.39 & 2.05$\times$   \\
MetaPruning~\cite{liu2019metapruning} &  & 76.60 &  75.40 &  1.20 & 2.05$\times$   \\	
PGMPF~\cite{cai2022prior} & & 76.01&75.11 & 0.90 & 2.20$\times$  \\
         Random Prune~\cite{li2022revisiting} & & 76.13 &  75.13 &  1.00 & 2.04$\times$   \\
		 GReg-1~\cite{wang2021neural} &  & 76.13 &   75.16 &  0.97 & 2.31$\times$   \\	
% 		& Real2Binary & 1/1 &  60.9 & 83.0  \\
       GReg-2~\cite{wang2021neural} &  & 76.13 &   75.36 &  0.77 & 2.31$\times$            \\	
      Ours &  & 76.13 &  \textbf{75.55} &  \textbf{0.58} & 2.31$\times$   \\	
	    \midrule
     		 LFPC~\cite{he2020learning}&  \multirow{4}*{ResNet-50} & 76.15  &  74.46 &   1.69 &  2.55$\times$  \\ % 
      GReg-1~\cite{wang2021neural} &  & 76.13 &   74.85 &  1.28 & 2.56$\times$   \\	
% 		& Real2Binary & 1/1 &  60.9 & 83.0  \\
       GReg-2~\cite{wang2021neural} &  & 76.13 &   74.93 &  1.20 & 2.56$\times$            \\	
              Ours &   & 76.13 &  \textbf{75.24} &  \textbf{0.89}  & 2.56$\times$   \\	
        \midrule
     		 IncReg~\cite{wang2019structured} &  \multirow{5}*{ResNet-50} & 75.60  &  71.07 &   4.53 &  3.00$\times$  \\ % 
      Taylor-FO \cite{molchanov2019importance}&  & 76.18 &   71.69 &  4.49 & 3.05$\times$   \\	
% CCEP~\cite{} \\
       GReg-1~\cite{wang2021neural} &  & 76.13 &   73.75 &  2.38 & 3.06$\times$            \\	
              GReg-2~\cite{wang2021neural} 
              &  & 76.13 &   73.90 &  2.23 & 3.06$\times$            \\	
              Ours 
              &  & 76.13 &   \textbf{74.26} &  \textbf{1.87} & 3.06$\times$   \\	
        \bottomrule
		\end{tabular}
  }
  }
\label{tab:imagnet}
\end{table}


% \begin{table*}[t]
% 	\centering
%  	\caption{
% 	{Acceleration comparison on ImageNet}. 
%  % \jvg{Table is very large. What is the added value of comparing to more than the top 3 per backbone? I would keep only 3 per backbone. } \jvg{If space is a concern; remove the "venue", "drop perc"} \jvg{why is speedup nog bold? Perhaps better to not use bold numbers at all? (ie: also not for accuracy; as the differences are so small) } \jvg{Note: Over emphasizing minor improvements (bold numbers/improved perc.) is annoying for reviewers} 
%  Speedup reflects the reduction on FLOPs. ResNet-34: 3.66GFlOPs, ResNet-50: 4.09GFLOPs.
%     }
% 	    \renewcommand{\arraystretch}{1.2}
% 		\setlength{\tabcolsep}{2.3mm}{
% 	    \resizebox{0.99\linewidth}{!}{
% 		\begin{tabular}[c]{lccccclccccc}
% 		\toprule			
%         \multirow{1}*{Method}  &  
%         \multirow{1}*{Venue}  & \multirow{1}*{Backbone} &  \multirow{1}*{Baseline Top-1 Acc (\%)} &   Pruned Top-1 Acc (\%) & {Top-1 Acc drop (\%) } & {Speedup}  \\\midrule
%    L1 (pruned-B)  ~\cite{li2017pruning} &  ICLR'17& \multirow{5}*{ResNet-34} & 73.23  &  72.17&   1.06 &  1.32$\times$  \\ % 
%       Taylor-FO~\cite{molchanov2019importance} & CVPR'19& & 73.31 &   72.83 &  0.48 & 1.29$\times$   \\	
% % 		& Real2Binary & 1/1 &  60.9 & 83.0  \\
%        GReg-1~\cite{wang2021neural} &ICLR'21& & 73.31 &   73.54 &  -0.23 & 1.32$\times$            \\	
%               GReg-2~\cite{wang2021neural} &ICLR'21& &  73.31  &   73.61 &  -0.30 & 1.32$\times$           \\	
%               Ours & CVPR'23& &  73.31  & \textbf{74.28}  &  \textbf{-0.97} & 1.32$\times$   \\	       \midrule		 IncReg~\cite{wang2019structured} & JSTSP'19 & \multirow{15}*{ResNet-50} & 75.60  &  72.47 &   3.13 &  2.00$\times$  \\ % \cmidrule(l){2-5}
%     	 SFP~\cite{he2018soft} & IJCAI'18 & & 76.15 &   74.61 &  1.54 &  1.72$\times$     \\	
% 	 HRank~\cite{lin2020hrank}& CVPR'20 &   &    76.15 &  74.98 &  1.17 & 1.78$\times$  \\ 	
% 		 Taylor-FO \cite{molchanov2019importance} & CVPR'19 & & 76.18 &  74.50 &1.68 &   1.82$\times$  \\
% 		Factorized~\cite{li2019compressing}& CVPR'19 & & 76.15 & 74.55 & 1.60 & {2.33$\times$}  \\
% 				 DCP~\cite{zhuang2018discrimination}& NIPS'18 & &  76.01 &  74.95 &  1.06   & 2.25$\times$   \\
% 		 CCP-AC~\cite{peng2019collaborative} & ICML'19 & &  76.15 &   75.32 & 0.83 & 2.18$\times$  \\
%    SRR~\cite{wang2021convolutional}
%    & CVPR'21 & & 76.13 &  75.11 &  1.02 & 2.27$\times$   \\	         AutoPruner~\cite{luo2020autopruner} & PR'20 & & 76.15 &  74.76 &  1.39 & 2.05$\times$   \\
% MetaPruning~\cite{liu2019metapruning} & CVPR'19 & & 76.60 &  75.40 &  1.20 & 2.05$\times$   \\	
% PGMPF~\cite{cai2022prior} & AAAI'22 && 76.01&75.11 & 0.90 & 2.20$\times$  \\
%          Random Pruning~\cite{li2022revisiting} & CVPR'22 & & 76.13 &  75.13 &  1.00 & 2.04$\times$   \\
% 		 GReg-1~\cite{wang2021neural} & ICLR'21 & & 76.13 &   75.16 &  0.97 & 2.31$\times$   \\	
% % 		& Real2Binary & 1/1 &  60.9 & 83.0  \\
%        GReg-2~\cite{wang2021neural} & ICLR'21 & & 76.13 &   75.36 &  0.77 & 2.31$\times$            \\	
%       Ours & CVPR'23 & & 76.13 &  \textbf{75.55} &  \textbf{0.58} & 2.31$\times$   \\	
% 	    \midrule
%      		 LFPC~\cite{he2020learning}& CVPR'20 & \multirow{4}*{ResNet-50} & 76.15  &  74.46 &   1.69 &  2.55$\times$  \\ % 
%       GReg-1~\cite{wang2021neural} & ICLR'21 & & 76.13 &   74.85 &  1.28 & 2.56$\times$   \\	
% % 		& Real2Binary & 1/1 &  60.9 & 83.0  \\
%        GReg-2~\cite{wang2021neural} & ICLR'21  & & 76.13 &   74.93 &  1.20 & 2.56$\times$            \\	
%               Ours &  CVPR'23  & & 76.13 &  \textbf{75.24} &  \textbf{0.89}  & 2.56$\times$   \\	
%         \midrule
%      		 IncReg~\cite{wang2019structured} & JSTSP'19 
%  & \multirow{5}*{ResNet-50} & 75.60  &  71.07 &   4.53 &  3.00$\times$  \\ % 
%       Taylor-FO \cite{molchanov2019importance}& CVPR'19  & & 76.18 &   71.69 &  4.49 & 3.05$\times$   \\	
% % CCEP~\cite{} \\
%        GReg-1~\cite{wang2021neural} & ICLR'21  & & 76.13 &   73.75 &  2.38 & 3.06$\times$            \\	
%               GReg-2~\cite{wang2021neural} 
%               & ICLR'21 & & 76.13 &   73.90 &  2.23 & 3.06$\times$            \\	
%               Ours 
%               & CVPR'23 & & 76.13 &   \textbf{74.26} &  \textbf{1.87} & 3.06$\times$   \\	
%         \bottomrule
% 		\end{tabular}
%   }
%   }
% \label{tab:imagnet}
% \end{table*}




\subsection{Results for ResNet-34/50 on ImageNet}

%\htor{this is a bit od and seems repeated after the ``convergence analysis'' given that the analysis above doesn't really show convergence but more computational effort - now here come final results, but the computational effort compared to the other methods is not clear?}

% \noindent \textbf{ResNet-34/50 on Imagenet.} 

We next evaluate our method with ResNet-34 and ResNet-50 on the large-scale ImageNet dataset.
We compare our results to previous pruning methods, including 
L1 Norm~\cite{li2017pruning}, TaylorFO~\cite{molchanov2019importance}, IncReg~\cite{wang2019structured}, SFP~\cite{he2018soft}, HRank~\cite{lin2020hrank}, Factorized~\cite{li2019compressing}, DCP~\cite{zhuang2018discrimination}, CCP-AC~\cite{peng2019collaborative}, LFPC~\cite{he2020learning}, GReg-1 and  GReg-2~\cite{wang2021neural},
SRR~\cite{wang2021convolutional},
MetaPruning~\cite{liu2019metapruning},
AutoPruner~\cite{luo2020autopruner},
PGMPF~\cite{cai2022prior} and
Random Pruning~\cite{li2022revisiting}.
% \yq{Adding the new add comparison}
For fair comparisons,
following~\cite{wang2021neural}, we use the official PyTorch ImageNet training example to assure that implementation details such as data augmentation, weight decay, momentum, etc.  match between methods. 

We first explore the behavior of our method by training ResNet-50 on ImageNet with the pruning setting corresponding to 3.06× speedup~\cite{wang2021neural} (see detail in \ref{Training_details}). 
In the top row of \fig{soft_evo}(b), we visualize the soft mask and L1 norm of 256 filters from layer 24 of the trained model. Note how all soft masks have converged to hard masks  and   that the L1 norms of the filters are  highly correlated with their corresponding mask values. 
% \bv{should we remove everything related to the correlation between L1-norm and mask, given that it's a (trivial) consequence of weight decay?}
In the bottom row of \fig{soft_evo}(b), we plot the validation accuracy of ResNet-50 during training.
We first use our method to prune the model for 90 epochs and, following previous work~\cite{wang2021neural},  finetune the pruned model for another 90 epochs. 
During the first stage, our method searches for the best architecture and reduces the importance of the pruned filters. After 90 epochs we can safely prune the filters without a large impact on the accuracy, in the star point we  test the accuracy for the derived sparse model before finetuning, after which finetuning  helps  to further improve the accuracy.
At the beginning of finetuning we observe a small accuracy drop since we use a larger learning rate to start with.


\tab{imagnet} gives  an overview of all comparisons. 
We group the methods with similar speedup together for easy comparison. 
We observe that our method consistently achieves
the best result among all approaches, for various speedup comparisons on different architectures.
On ResNet-34, our method improves the baseline (unpruned) model by 0.97\% accuracy.
Previous work~\cite{hoefler2021sparsity} explained how pruning
can improve generalization performance to improve accuracy  for unseen data drawn from the same distribution.
Such improved accuracy after pruning has been observed in earlier work \cite{he2017channel}, but has been more apparent for smaller datasets like CIFAR. In agreement with~\cite{wang2021neural} we also observe improvements over the baseline accuracy on the much more
challenging ImageNet benchmark. 
With larger speedups, the advantage of our method becomes more obvious. For example, our method outperforms
Taylor-FO~\cite{molchanov2019importance}  by 1.05\% top-1 accuracy at the $2.31\times$ setting, while at $3.06\times$,
ours is better by 2.57\% top-1 accuracy.
Previous work has made considerable progress defining importance scores based on the networks weights ~\cite{li2017pruning} ~\cite{he2020learning}. In contrast to those studies our method learns the importance scores used to prune the network in an end-to-end fashion. Our results indicate this can improve the accuracy of pruned networks.

\RVC{
\noindent \textbf{Global Sparsity for MobileNetV2.}
Thus far we have focused on normal convolutions, but networks based on depthwise convolutions may be harder to prune. In~\tab{gloabalsparsity}, we compare to ChipNet~\cite{tiwari2021chipnet} using the global sparsity ratio for the lightweight  MobileNetV2 architecture on CIFAR-10/100.
Learning with a global sparsity ratio may distribute different sparsity ratios across layers, while respecting the preset sparsity across the network.
For both datasets, we rerun the experiments of ChipNet using 
its released hyperparameters and training settings.
Under different sparsity ratios, our method consistently outperforms ChipNet.  


\noindent \textbf{Unstructured Pruning on ImageNet.}
Thus far we focused on  structured filter pruning, but previous studies have also explored unstructured pruning. In \tab{imagnet_unstru}, we show that our method can also be applied to unstructured pruning use cases. 
Our method compares favorably to other advanced unstructured pruning methods for ResNet-50 on ImageNet.


We also further extend our method to general budgeted pruning with e.g. a certain FLOP budget (see details in \ref{flopslatency}).



}
% \begin{figure*}[t]
% \centering
% \begin{tabular}{ccc}
%     \includegraphics[width=0.46\textwidth]{figure/soft_mask_visual/figure_index48_epoch1.pdf} &
%     % \includegraphics[width=0.295\textwidth]{iclr2023/figure/soft_mask_visual/figure_index48_epoch5.pdf} &
%         \includegraphics[width=0.46\textwidth]{figure/soft_mask_visual/figure_index48_epoch120.pdf}
%     \end{tabular}
%     \caption{ \small
%  The x-axis is the filter index and y-axis shows the  values of  our soft mask and the L2 norm of  filters.     We use a fixed regularization hyperparameter $\varepsilon = 1$. 

%  % As training, our soft mask converges to the original optimal sparse solution.
%  % At starting, all filters have similar importance yet L2 norm, then the importance of pruned filters gradually decreased to zero thus we can safely prune them. 
%  In early training phases (left), all filters have similar L2 norms and soft masks.  In later training phases the soft masks have converged to hard
% masks, which highly correlate with the L2 norms of the filters. Thus we can safely prune them.
%     }
%  \label{fig:decision_bound}
% \end{figure*}




% Pr = 0.9
% epsilon = 100:  87.29
% epsilon = 10:  88.99
% epsilon = 1:  89.75
% epsilon = 0.1:  88.88
% epsilon = 0.01:  88.78

% \begin{table*}[t]
% 	\centering
%  	\caption{ VGG-19 on CIFAR100:  
% 	Accuracy comparison with  GReg-1 \cite{wang2021neural},  Each experiment is repeated 3 times with random initialization, mean and std of the accuracies our reported.
%     }
% 	\renewcommand{\arraystretch}{1.3}
% 	\resizebox{0.99\linewidth}{!}{
% 	 \setlength{\tabcolsep}{3.5mm}{
% 	   	\begin{tabular}{lcccccc}
%     	\toprule
% 		 Pruning ratio (\%) & 50  & 60 &  70  & 80 & 90 \\
%    		 Sparsity (\%) / Speedup & 74.87/3.60$\times$  & 84.00/5.41$\times$  &  90.98/8.84$\times$   & 95.95/17.30$\times$  & 98.96/44.22$\times$  \\
%       \midrule		
% 		 $L_1$+one-shot (Acc. \%)~\cite{li2017pruning} & 71.49$\pm$0.14  & 70.27$\pm$0.12 &  66.05$\pm$0.04 &  61.59$\pm$0.03 &  51.36$\pm$0.11 \\
% 		 GReg-1 (Acc. \%)~\cite{wang2021neural}  & 71.50$\pm$0.12  & 70.33$\pm$0.12 &  67.35$\pm$0.15 &  63.55$\pm$0.29 &  57.09$\pm$0.03 \\ 		
% 		  Ours (Acc. \%) & \textbf{71.56$\pm$0.19}
%     & \textbf{70.41$\pm$0.06}
%     &   \textbf{67.74$\pm$0.13}
%     &   \textbf{63.98$\pm$0.25}
%     &   \textbf{57.21$\pm$0.09}
%     \\	
% 	   \bottomrule
% 	\end{tabular}
% 	}}
% 	\label{tab:vgg_cifar100}
% \end{table*}




%-------------------------------------------------








==> followup.tex <==
\section{Follow up experiments} \label{followup
}
Additional experiments and other fixes that we plan to have ready during the rebuttal period.
\subsection{Unstructured pruning}
We apply our method for unstructured pruning on CIFAR-10 and ImageNet datasets

\noindent \textbf{CIFAR-10 with ResNet-56.}
Baseline accuracy (no pruning) is 93.36\%. We compare the performance of independent learnable score and dependent score where network weights as scores; compare difference using dual space and original space of optimizing dual variables; and compare using 2nd order and 1st order gradients where 1st order means we do not count the gradients of updated dual variables w.r.t scores (envelope theorem).
\begin{itemize}
    \item Pruning ratio 90\% + $\varepsilon = 1$ + Dual space:  \\
    \textit{i)}. Independent score-- 
    
    92.26\% (no finetuning) +92.42 \% (with finetuning).  \\
    \textit{ii)}. Dependent score -- 
    
    92.34 \% (no finetuning) + 92.57\% (with finetuning).
    \item Pruning ratio 90\% + $\varepsilon = 1$ + Original space:  \\
    \textit{i)}. Independent score + 2nd order -- 
    
    92.22\% (no finetuning) + 92.55\% (with finetuning).  \\
    \textit{ii)}. Independent score + 1st order -- 
    
    92.01\% (no finetuning) + 92.65\% (with finetuning).
\end{itemize}
\noindent \textbf{ImageNet  with ResNet-50.} See \tab{imagnet_unstru}






\subsection{Iterative pruning + Structured filter pruning}
TODO: to show our method works well with iterative pruning

\subsection{Combine structured filter pruning techniques}
TODO: build a strong baseline






==> method.tex <==
\section{Old: Differentiable Transportation Pruning}
\label{methods}

% \yq{TODO: Toy Example}

\bv{NON-MATH EXPLANATION OF METHOD: In filter pruning we remove those filters that contribute less to network accuracy. We would therefore like to find a mapping between the filters on the one hand, and a binary mask that signals if we can remove a filter or not on the other hand. Given a predetermined pruning rate, we can phrase this mapping problem in terms of optimal transport: We start from a discrete uniform distribution over the filters and aim to transform this distribution into a Bernouilli distribution of masks that reflects the pruning rate. To transform between the two distributions optimal transport moves probability mass from one distribution to the other, but moving probability mass from one location to the other comes at a cost. In our method the transportation cost is optimized by minimizing the distance between a binary mask variable that follows the above Bernouilli distribution and a learned importance score. In other words, we train importance scores to be higher for important filters and lower for filters that can be removed.  }


We describe the
% training-aware pruning
Differentiable Transportation (DT) Pruning algorithm using a discrete binary mask
in general form in Section \ref{discretemasked}, 
where a binary mask
parameterized by a learnable parameter vector  is trained for pruning. % with model parameters
We then introduce a simple
 entropic regularized transportation approximation 
for our discrete mask which leads to a differentiable bilevel-learning objective 
for the optimization of the dual multipliers and model variables \jvg{Difficult to understand at this point of the text as these terms have not been explained} (Section \ref{DifferentiableTransportation}). Finally,  we propose an
approximation technique to make the algorithm computationally feasible and efficient (Section \ref{Approximate_optimization}).


\subsection{Discrete Masked Pruning}
\label{discretemasked}
Given $\mathbf{s} \in \mathbb{R}^{n, +}_0$ \jvg{I dont understand this notation; why is it not $\mathbb{R}^{n}$ ? } as an  importance score vector, $\mathbf{m}(\mathbf{s}) \in \{0, 1\}^n$ denotes a discrete binary mask parameterized by $\mathbf{s}$  and $n$ is the dimensionality of binary mask. With  a predefined  pruning rate $p$ and let $\bf{1}_n$ \jvg{$\bf{1}_n$ ?} denote a vector with $n$ ones, we formulate the training-aware pruning as a discrete masked pruning problem:
 \begin{equation}
\begin{split}
& \mathop{\min}_{\mathbf{s}, \mathbf{w}}\ \ 	\mathcal{L}_\text{train} \big(\mathbf{m}(\mathbf{s}), \mathbf{w}\big),
 \\
 & \ \ \ \text{s.t.} \ \ \   {\bf{1}_n^{\mathsf{T}} \mathbf{m}}/{n}  = p, 
\  \   \mathbf{m} \in \{0, 1\}^n,
\end{split}
\label{eq:formulate_pruning}
\end{equation}
\jvg{what is $\mathcal{L}$?} \jvg{should it be arg min?}  \jvg{How can you divide m by n? Is m not a function? Do you mean $m(s)$? } \jvg{if $1_n$ is a vector, then $1_n^t$ is a column vector, but you probably mean a row vector here? and then transpose m?} \jvg{instead of multiplying with a vector of 1s, which needs a symbol to be defined; is it not simpler to just say that 1/n sum(m(s)) = p ?}
where $\mathbf{w}$ is the model parameters. 
% In fine-grained sparsity learning, $\mathbf{w}$ has equal dimensionality with $\mathbf{m}$.
The introduced binary mask
encodes the connection information \jvg{what is a connection? (try to not introduce new terms)}, where a zero element 
% in $\mathbf{m}$
indicates a pruned connection. 
This formulation is applicable to a variety
of sparsity methods including  unstructured and  structured
pruning. 
Objective (\ref{eq:formulate_pruning})   aims to train the mask 
 jointly with the model parameters  for pruning. \jvg{the mask is not applied? Or is that done in the loss term L? }
% Learning the binary mask  is of core practical importance
% in optimizing  \eq{formulate_pruning}.

Learning the binary mask 
in \eq{formulate_pruning}  
% is simply a top-$k$ operator of importance score  where top $p$ percent elements of sorted
% $\mathbf{s}$ are assigned to $1$ and  the remaining elements are assigned to $0$.
% This top-$k$ operator 
can be parameterized in terms of the  solution of
an optimal transport problem~\cite{xie2020differentiable, li2021deep, ramanujan2020s}. 
Optimal transport (OT)
aims to find a minimal transportation cost plan between  two probability distributions. We use OT to align the importance score   distribution with the discrete binary mask distribution. \jvg{why is this useful? What does the importance score do? } \jvg{What distributions are those?}

\jvg{Start with a non-math motivation; ie: explain what you will do in English first, and then use the math to make it precise} We define two discrete measures  $\mathbf{a} = \sum_{i = 1}^n \mathbf{a}_i \delta_{\mathbf{s}_i}$ and 
$\mathbf{b} = \sum_{j = 1}^2 \mathbf{b}_j \delta_{\mathbf{m}_j}$ supported on $\{\mathbf{s}_i\}_{i = 1} ^n$ and $\{\mathbf{m}_j\}_{j = 1} ^2 = \{0, 1\}$ respectively \jvg{isnt m a function? Do you mean $m(s_j)$?} \jvg{you index the dirac function also with m; and if m is a function, than this is weird.},  where $\delta_x$ is the Dirac function at location $x$, the $\mathbf{a}_i$ and $\mathbf{b}_j$ are the probability mass \jvg{where does this probability come from?} associated with the corresponding location $\mathbf{s}_i$ and  $\mathbf{m}_j$. Particularly, a binary mask variable only has two locations $\mathbf{m}_1$ and $\mathbf{m}_2$, with the corresponding mass $\mathbf{b}_1$ and $\mathbf{b}_2$.
Given the pruning rate $p$, 
% The empirical distribution is simply the  counting numbers of value in that position, then 
we have $\mathbf{a} = \mathbbm{1}_n / n$  \jvg{why? you get a vector of length n with constant values 1/n ?} and $\mathbf{b} = [p, 1-p]^{\mathsf{T}}$, where $\mathbb{P}( \{\mathbf{s}_i\}) = 1/n$ and $\mathbb{P}( \{0\}) = p$. The corresponding
optimal transport cost \jvg{between which distributions?} can be formulated as: \bv{here it must be argmin because you want the argument that minimizes the function, same comment applies below: \yq{I still can not get why it is argmin:)}}
  \begin{equation}
\mathbf{P}^*= \mathop{\min}_{\mathbf{P} \in\mathcal{U}(\mathbf{a}, \mathbf{b})}	\left \langle \mathbf{C}, \mathbf{P}\right \rangle, 
% \ \ \text{s.t.} \ \ 
% \mathbf{P} 
%  \mathbbm{1}_2 = \mathbf{a}, \  \mathbf{P}^\mathsf{T} \mathbbm{1}_n = \mathbf{b}, 
\label{eq:opt}
\end{equation}
where $\mathcal{U}(\mathbf{a}, \mathbf{b}) = \{\mathbf{P}\in \mathbb{R}^{n \times 2}: \mathbf{P} 
 \mathbbm{1}_2 = \mathbf{a}, \  \mathbf{P}^\mathsf{T} \mathbbm{1}_n = \mathbf{b}\}$ \jvg{I do not understand this} and 
$\mathbf{P}$ is the general probabilistic coupling matrix
% that indicates how much mass is transported to
% push distribution $\mathbf{a}$ towards distribution $\mathbf{b}$ 
and 
$\mathbf{C} \in \mathbb{R}^{n \times 2}$ is the cost function matrix.
% whose element  denotes the
% non-negative cost to move a probability mass from distribution $\mathbf{u}$ to $\mathbf{v}$.
When the cost is defined as the squared Euclidean distance, 
OT is
referred to as a 2-Wasserstein distance. The elements  of  the cost matrix are denoted as $\mathbf{C}_{i1} = \mathbf{s}_i^2$  and $\mathbf{C}_{i2} = (\mathbf{s}_i - 1)^2$ for $i = 1, 2,...,n$. 
The optimal  $\mathbf{P}^*$ is referred to as the optimal transport plan which can be computed with linear programming.
In our binary mask case,  the optimal transport plan  in  \eq{opt}  is obtained by a simple top-k operator~\cite{xie2020differentiable}:
 \begin{equation}
\mathbf{P}^*_{\sigma_i, 1}  =
\begin{cases}
1/n,  & \mathrm{if \  } i \leq n \cdot p \\
0, & \mathrm{otherwise}
\end{cases}, 
\mathbf{P}^*_{\sigma_i, 2} = 
\begin{cases}
0, & \mathrm{if \  } i \leq n \cdot p \\
1/n, & \mathrm{otherwise}
\end{cases}
\label{eq:hardassign}
\end{equation}
 with $\sigma$  being the sorting permutation, \ie \ $\mathbf{s}_{\sigma_1} < \mathbf{s}_{\sigma_2} <\cdot\cdot\cdot < \mathbf{s}_{\sigma_n}$. 
 Given  $\mathbf{P}^*$, the binary mask can be parameterized by the optimal transport plan: \bv{:here we just take the second column of P and multiply by n, so would be simpler to write that}
 \begin{equation}
\mathbf{m} = n\mathbf{P}^*\cdot[0, 1]^{\mathsf{T}}.
\label{eq:optsolution}
\end{equation}


The task of optimizing binary mask in \eq{formulate_pruning} therefore reduces to learning the optimal transport plan in \eq{opt}.
However, the optimal transport plan in \eq{hardassign} is non-differentiable with respect to the learnable importance score $\mathbf{s}$, and immediately pruning with a discrete mask   may hurt performance. 
Therefore, in the following, 
we apply convex relaxation
of the transportation plan learning via entropic regularization, and propose a simple method to gradually approach the discrete optimal solution.
% \yq{TODO}
% To jointly learn the binary mask and the model parameters in \eq{formulate_pruning}  via stochastic gradient descent(SGD), in the following we relax the transportation plan 
% via a simple
% relative entropic regularized transportation approximation 
% by proximal point iterations.
% To make the optimal transport plan continuous, in the following we relax
% the:
% In the following we propose a simple
% relative entropic regularized transportation approximation 
% by proximal point iterations to 
% This makes it difficult to train
% binary networks via stochastic gradient descent(SGD)





% Learning the binary mask  is of core practical importance
% in optimizing  \eq{formulate_pruning}.
% For example, the weight connections in fine-grained sparsity learning  are $\mathbf{m} \odot\mathbf{w}$ with $\odot$ denotes element wise product.





\subsection{Differentiable Transportation Relaxation and Optimization} 
% \yq{Define the soft mask somewhere }
\label{DifferentiableTransportation}
Define the discrete entropy of a coupling matrix $\mathcal{H}(\mathbf{P}) = -\sum_{ij}\mathbf{P}_{ij}(\text{log}(\mathbf{P}_{ij}) - 1)$, an entropic regularization is used  to  obtain approximate solutions to the original transport problem in \eq{opt}:
   \begin{equation}
\mathbf{P}^{*}_{\varepsilon}= \mathop{\min}_{\mathbf{P} \in\mathcal{U}(\mathbf{a}, \mathbf{b})}	\left \langle \mathbf{C}, \mathbf{P}\right \rangle - \varepsilon \mathcal{H}(\mathbf{P}).
\label{eqn:entropyopt2}
\end{equation}
This objective is an $\varepsilon$-strongly convex function \jvg{why is it now convex?} which has a unique optimal solution. 
As $\varepsilon\to0$ the unique solution $\mathbf{P}_{\varepsilon}$ of (\ref{eqn:entropyopt2}) converges to the original optimal sparse solution of (\ref{eq:opt}). 
By introducing two dual variables $\mathbf{f}\in \mathbb{R}^{n}$ and $\mathbf{g}\in \mathbb{R}^{2}$ for each marginal constraint in  $\mathcal{U}(\mathbf{a}, \mathbf{b})$, 
the Lagrangian of (\ref{eqn:entropyopt2}) is optimized which results for 
 an optimal $\mathbf{P}_{\varepsilon}$ coupling to the regularized problem, in the expression:
%     \begin{equation}
% \mathbf{P}^{\varepsilon}_{ij} = e ^{{\mathbf{f}_i}/{\varepsilon}} e ^{-{\mathbf{C}_{ij}}/{\varepsilon}}e ^{{\mathbf{g}_j}/{\varepsilon}}.
% \label{eq:lagrange}
% \end{equation}
    \begin{equation}
\mathbf{P}_{\varepsilon} = e ^{{\mathbf{f}}/{\varepsilon}} \odot e ^{-{\mathbf{C}(\mathbf{s})}/{\varepsilon}} \odot e ^{{\mathbf{g}}/{\varepsilon}}.
\label{eq:lagrange}
\end{equation}
where  $\odot$ is element wise product (See details in \ref{Optimal_coupling}).
Note that the $\mathbf{P}_{\varepsilon}$ in \eq{lagrange} is differentiable with respect to $\mathbf{s}$. 
After relaxation, our goal is to jointly learn the dual
variables $\mathbf{f}$, $\mathbf{g}$ and the model variables $\mathbf{s}$, $\mathbf{w}$, 
where the dual variables are optimized by minimizing the regularized optimal transport distance in \eqn{entropyopt2}  
which is equivalent to maximizing its dual problem denoted as   $\mathcal{L}_\text{dual}^{\varepsilon} (\mathbf{f}, \mathbf{g}, \mathbf{s}) = \left \langle \mathbf{f}, \mathbf{a}\right \rangle
+ \left \langle \mathbf{g}, \mathbf{b}\right \rangle
- \varepsilon \left \langle e ^{{\mathbf{f}}/{\varepsilon}},  e ^{-{\mathbf{C}{(\mathbf{s})}}/{\varepsilon}} \cdot e ^{{\mathbf{g}}/{\varepsilon}}\right \rangle$ (See details in \ref{Dual_problem}),
and the model variables are obtained by minimizing the training loss, \eg, \  cross entropy loss denoted as $\mathcal{L}_\text{train}$. 




This implies a
\textit{bilevel optimization problem} \jvg{what is that? Give a citation, and/or explain in a few words} with model variables $\mathbf{s}$, $\mathbf{w}$ as the upper-level variables and  dual variables $\mathbf{f}$,  $\mathbf{g}$ as the lower-level variables. We rewrite the original problem in \eq{formulate_pruning}  as the following bilevel optimization problem:
\begin{align}
& \mathop{\min}_{\mathbf{s}, \mathbf{w}}\ \ 	\mathcal{L}_\text{train} \Big(\mathbf{m} \big(\mathbf{P}^*_{\varepsilon}(\mathbf{s})\big), \mathbf{w}\Big),
 \label{eq:upper} \\
 & \ \ \  \text{s.t.} \ \ \  \mathbf{P}^*_{\varepsilon}(\mathbf{s})  =  	\mathop{\max} \nolimits_{\mathbf{f},  \mathbf{g}}  \   \mathcal{L}_\text{dual}^{\varepsilon} (\mathbf{f}, \mathbf{g}, \mathbf{s}),\label{eq:lowerl} 
	\end{align}
% \begin{align}
% & \mathop{\min}_{\mathbf{s}, \mathbf{w}}\ \ 	\mathcal{L}_\text{train} (\mathbf{m}^*_{\varepsilon} (\mathbf{f}^*(\mathbf{s}), \ \mathbf{g}^*(\mathbf{s}), \mathbf{s}), \mathbf{w}),
%  \label{eq:upper} \\
%  & \ \ \  \text{s.t.} \ \ \  (\mathbf{f}^{*}(\mathbf{s}), \ \mathbf{g}^{*}(\mathbf{s}))_{\varepsilon}  =  	\mathop{\argmin} \nolimits_{\mathbf{f},  \mathbf{g}}  \   \mathcal{L}_\text{reopt}^{\varepsilon} (\mathbf{f}, \mathbf{g}, \mathbf{s}, \mathbf{w}),\label{eq:lowerl} 
% 	\end{align}
where the mask $\mathbf{m}_{\varepsilon}$  in (\ref{eq:upper}), dubbed as soft mask, is computed with (\ref{eq:optsolution}) and (\ref{eq:lagrange}) after obtaining optimal dual variables from (\ref{eq:lowerl}) that can be solved  with Sinkhorn's iterative algorithm~\cite{cuturi2013sinkhorn} (details in \ref{sinkhorn}). 

Similar nested formulations have found their use in differentiable neural architecture search~\cite{liu2019darts, cai2019proxylessnas} and
gradient-based hyperparameter optimization \cite{maclaurin2015gradient, franceschi2018bilevel}. 
In contrast, our bilevel formulation adds an  additional hyperparameter $\varepsilon$ to decay, which makes the problem harder to optimize. 
 Firstly, per mini-batch the inner optimization  in \eq{lowerl} needs to perform Sinkhorn's iterative algorithm for hundreds of iterations to converge, which is expensive and computationally inefficient; 
furthermore, in the back-propagation pass, the gradient of optimal coupling $\mathbf{P}^*_{\varepsilon}(\mathbf{s})$ in \eq{upper}
 with respect to the importance scores  $\mathbf{s}$ needs to perform automatic differentiation~\cite{paszke2017automatic} back into these inner Sinkhorn iterations \htor{what does ``perform AD back into an interation'' mean?} which is difficult to obtain; 
 and last the decaying strategy of the additional hyperparameter $\varepsilon$
 is difficult to tune. 
In the next section,
% we propose an approximation method 
% to make
% the algorithm computationally  efficient and  make the decaying schedule of hyperparameter performed in an automatic manner.
we propose an approximation method that makes the algorithm more computationally  efficient, and automatically decays the hyperparameter  $\varepsilon$.



\begin{algorithm}
\caption{Differentiable Transportation Pruning}\label{alg:algrithorm}
\begin{algorithmic}
\Require Probabilities: $\mathbf{a}={\mathbbm{1}_n}/{n}$, $\mathbf{b} = [p, 1-p]^{\mathsf{T}}$ on supports: $\{\mathbf{s}_i\}_{i = 1} ^n$, $\{\mathbf{m}_j\}_{j = 1} ^2$, Initialization: $\varepsilon$, 
 $\mathbf{g}^{(1)} \gets \mathbbm{1}_2 $, $\mathbf{P}^{(1)} \gets \frac{1}{n}\mathbbm{1}_n \mathbbm{1}_2^{\mathsf{T}}$,
  Weights: $\mathbf{w}$, Training loss: $\mathcal{L}_\text{train}$, 
  Training iterations: $L$,  Learning rate:  $\alpha$
 \For  {$l = 1, 2,..., L$}
 % $\mathbf{C}_{i1} = \mathbf{s}_i^2$  and $\mathbf{C}_{i2} = (\mathbf{s}_i - 1)^2$
% points  $n \geq 0$
% \Ensure $y = x^n$
\State Cost matrix $\mathbf{C}$ with element $\mathbf{C}_{ij} = (\mathbf{s}_i - \mathbf{m}_j)^2$
\State  Gibbs kernel $\mathbf{K} = e^{-\frac{\mathbf{C}}{\varepsilon}} \odot \mathbf{P}^{(\ell)}$
\State Update dual variables  with \eq{gvaraible} for one step:
\State \ \ \ \ \ \ \
 $\mathbf{f}^{(\ell+1)} = \varepsilon \ \text{log} \ \mathbf{a}  - \varepsilon \ \text{log} \ (\mathbf{K}e^{\mathbf{g}^{(\ell)}/\varepsilon} )$
\State \ \ \ \ \ \  \
 $\mathbf{g}^{(\ell+1)} = \varepsilon \ \text{log} \ \mathbf{b}  - \varepsilon \ \text{log} \ (\mathbf{K}^{\mathsf{T}}e^{\mathbf{f}^{(\ell + 1)}/\varepsilon} )$
\State Compute $\mathbf{P}^{(\ell+1)} = e^{{\mathbf{f}^{(\ell+1)}}/{\varepsilon}}  \odot \mathbf{K}  \odot e^{{\mathbf{g}^{(\ell+1)}}/{\varepsilon}}$ 
% in \eq{decayauto}
% \State Update model  varaibels $\mathbf{w}$ and $\mathbf{s}$ using stochastic
% gradient descent (SGD):
\State Gradients  w.r.t. model variables,  $\nabla_\mathbf{s}\mathcal{L}_\text{train}$; 
% in \eq{approximate}
 $\nabla_\mathbf{w}\mathcal{L}_\text{train}$    
\State   Update model variables with SGD:
\State \ \ \ \ \ \  \ $\mathbf{s} = \mathbf{s} - \alpha   
\nabla_\mathbf{s}\mathcal{L}_\text{train} $; \ \  $\mathbf{w} = \mathbf{w} - \alpha   \nabla_\mathbf{w}\mathcal{L}_\text{train}$
% \State   Update model weights $\mathbf{w} = \mathbf{w} - \alpha   \nabla_\mathbf{w}\mathcal{L}_\text{train}$
 \EndFor 
 \State 
 Derive the pruned architecture based on soft mask $\mathbf{m} = n\mathbf{P}^{(L)}\cdot[0, 1]^{\mathsf{T}}$ in \eq{optsolution} for finetuning.
\end{algorithmic}
\end{algorithm}





\begin{figure*}[t]
\centering
\begin{tabular}{ccc}
     \includegraphics[width=0.43\textwidth]{figure/scores_all/Toghether3maskIter_independencescore1.pdf} &
         \includegraphics[width=0.543\textwidth]{figure/scores_all/imagenet_acc_mask1.pdf}  
         \\  
         \ \ \ \small{(a) 
  On CIFAR10}  &
  \small{(b) On ImageNet}
  
    % \includegraphics[width=0.295\textwidth]{iclr2023/figure/soft_mask_visual/figure_index48_epoch5.pdf} &
%         \includegraphics[width=0.32\textwidth]{iclr2023/figure/scores_all/Iter_independencescore.pdf} 
% \includegraphics[width=0.33\textwidth]{iclr2023/figure/scores_all/Iter_L2norm.pdf}
    \end{tabular}
    \caption{ 
    Convergence analysis experiments.
   \textit{(a).} 
   Evolution  of the soft masks associated with three filters from
    ResNet56 trained on CIFAR10 with $\varepsilon = 1$.  
 % During training our soft mask converges to a discrete hard mask solution. 
 Early in training our method explores different filter compositions.  In later training phases the soft masks have converged to hard
masks. For each mask, the soft mask, importance score and L1 norm of the respective filter are correlated. \htor{why do all scores go towards zero (not corr with masks at 1!)}
  \textit{(b).} 
    Experiments with ResNet50 on ImageNet with $\varepsilon = 0.25$.  
 % During training our soft mask converges to a discrete hard mask solution. 
  After training the soft mask has converged to a discrete hard mask solution. 
The L1 norms of the filters are highly correlated with the soft masks \htor{can we put L1 on a different scale on the right side so one can see the corr clearer?}. Bottom: Validation accuracy during training with differential transportation pruning and during finetuning. 
The star point shows the test accuracy for the derived pruned architecture by our soft mask before finetuning. \htor{maybe annotate the regions in the plot?}
( [TODO: ADD A AND B, REPOSITION LEGENDS]
 % As training, our soft mask converges to the original optimal sparse solution.
 % At starting, all filters have similar importance yet L1 norm, then the importance of pruned filters gradually decreased to zero thus we can safely prune them. 
    }
 \label{fig:soft_evo}
\end{figure*}

%  \begin{equation}
% \begin{split}
% & \mathop{\min}_{\mathbf{s}, \mathbf{w}}\ \ 	\mathcal{L}_{train} (\mathbf{f}^*(\mathbf{s}), \ \mathbf{g}^*(\mathbf{s}), \mathbf{s}, \mathbf{w}),
%  \\
%  & \ \ \  \text{s.t.} \ \ \  \mathbf{f}^*(\mathbf{s}), \ \mathbf{g}^*(\mathbf{s})  =  	\mathop{\argmin} \nolimits_{\mathbf{f},  \mathbf{g}}  \   \mathcal{L}_{breg} (\mathbf{f}, \mathbf{g}, \mathbf{s}, \mathbf{w}).
% 	\end{split}
% \label{eq:bilevelgradienet}
% \end{equation}
\subsection{Approximate Bilevel Optimization}
\label{Approximate_optimization}
To solve the bilevel problem, we  approximate $\mathbf{P}^*_{\varepsilon}(\mathbf{s})$ in \eq{lowerl} using  only a single training \htor{is this really ``training'' (usually backprop) or just a solver iteration?}
step, \ie, without 
training the inner optimization until convergence. Given the $\ell$-th mini-batch update step, we have:
 \begin{equation}
\begin{split}
& \nabla_\mathbf{s}	\mathcal{L}_\text{train} \Big(\mathbf{m} \big(\mathbf{P}^*_{\varepsilon}(\mathbf{s})\big), \mathbf{w}\Big)
\\
 \approx &\nabla_\mathbf{s}  \mathcal{L}_\text{train} \Big(\mathbf{m} \big(\mathbf{P}^{(\ell+1)}_\varepsilon(\mathbf{s})\big), \mathbf{w}\Big),
\end{split}
\label{eq:approximate}
\end{equation}
where $\mathbf{P}^{(\ell+1)}_\varepsilon(\mathbf{s})$ is obtained for a single update step.  Similar, the techniques have been used  in architecture search~\cite{liu2019darts}, gradient based hyperparameter tuning~\cite{luketina2016scalable}, meta-learning for model transfer~\cite{finn2017model} and unrolled generative adversarial networks~\cite{metz2016unrolled}.


To enhance the convergence guarantee  using just a single Sinkhorn inner  iteration, 
we  use generalized proximal point iteration
 based on Bregman divergence (details in \ref{Bregman}). 
 % \yq{TODO: explained}\cite{parikh2014proximal, rockafellar1976monotone}. 
 Using this technique, \cite{xie2020fast} have shown both theoretically and empirically
that a single
Sinkhorn inner iteration is  sufficient to converge to \eq{lowerl} under a large range of fixed $\varepsilon$, we therefore compute  $\mathbf{P}^{(\ell+1)}_\varepsilon(\mathbf{s})$ in \eq{approximate} as:
  \begin{align}
\mathbf{P}^{(\ell+1)}_\varepsilon(\mathbf{s}) &= e ^{\frac{\mathbf{f}^{(\ell+ 1)}}{\varepsilon}}  \odot \big(e^{-\frac{\mathbf{C}(\mathbf{s})}{\varepsilon}} \odot \mathbf{P}^{(\ell)}\big)  \odot e ^{\frac{\mathbf{g}^{(\ell + 1)}}{\varepsilon}}.
\label{eq:decayauto}
\end{align}
Let $\mathbf{K} = e^{-{\mathbf{C}(\mathbf{s})}/{\varepsilon}} \odot \mathbf{P}^{(\ell)}$ denote the Gibbs kernel in the Sinkhorn algorithm, where the dual variables are updated for a single Sinkhorn iteration with block coordinate ascent (details in \ref{sinkhorn}): 
\begin{align}
  &\mathbf{f}^{(\ell+1)} = \varepsilon \ \text{log} \ \mathbf{a}  - \varepsilon \ \text{log} \ (\mathbf{K}e^{\mathbf{g}^{(\ell)}/\varepsilon} ); \\  &\mathbf{g}^{(\ell+1)} = \varepsilon \ \text{log} \ \mathbf{b}  - \varepsilon \ \text{log} \ (\mathbf{K}^{\mathsf{T}}e^{\mathbf{f}^{(\ell + 1)}/\varepsilon} ). \label{eq:gvaraible} 
	\end{align}
 As shown in \cite{peyre2019computational, schmitzer2019stabilized} the proximal point iterations iteratively apply the Sinkhorn’s algorithm with a
$e^{-\frac{\mathbf{C}}{\varepsilon/\ell}}$
kernel, \ie, \ with a decaying regularization parameter $\varepsilon/\ell$, therefore it can perform  an automatic decaying schedule on the regularization as $\ell\to\infty$ to gradually approach the optimal discrete plan of the original objective (\ref{eq:formulate_pruning}). Thus the proximal point iteration can be seen as iterative Sinkhorn (details in \ref{proximal_sinkhorn}). 

  The  gradient of \eq{decayauto}  with respect to the importance score 
  is easy to compute using the chain rule, 
  thus we can simply obtain the approximate gradient with respect to the importance score in \eq{approximate} for training importance score by  stochastic gradient descent (SGD). 
   The model weights $\mathbf{w}$ are also trained with SGD. 
   Our method results in fast training and converges quite well as shown by our experiments in Section \ref{exp}. We outline the iterative training procedure   in \alg{algrithorm}.
   
\htor{I would love to see a complete overview/viewgraph of the whole method and its steps/approximations - maybe with some nice viz. Could also go right into the introduction as poster child.}













% \subsection{Deriving Discrete Architecture}

% \yq{TODO}




==> new_delete.tex <==
\section{Rebuttal} \label{rebut
}

We thank the reviewers for their thoughtful comments and suggestions. We have clarified and performed additional analyses where needed, all of which have strengthened the manuscript.

\textbf{Budget-aware pruning (rev oGyB, gUFv, TZHc)}
We cannot directly compare our ImageNet results to studies employing FLOP and latency based budget-aware pruning techniques: First, these techniques use different objective functions, based on e.g. FLOPs or latency vs. our filter budget. Second, these techniques prune across all network filters. For fair comparisons with ~\cite{wang2021neural}, we used fixed layer-wise pruning rates, which strongly constraints the search space. Third, the baseline models and hyper-parameter settings are different in these studies. However, we performed additional analyses comparing our work to ChipNet under different global filter budgets (Table2) for MobileNetV2 on CIFAR-10/100, and under different FLOPs budgets (Table3) for WideResNet-26 for CIFAR-100. For the latter we formulate the FLOPs budget pruning as a learnable sparsity allocation problem. For both budget types our method compares favorably to CHIPNet. We describe the method on page \bv{TODO: add table refs and refer to main text for method description}

\textbf{Results for MobileNetV2 (rev oGyB, yBMK)}
In Table2, we added an experimental comparison on MobileNetV2 for different budgets types on CIFAR-10 and CIFAR-100, showing that our method works well on lightweight architectures. These results have been added to the main manuscript. \bv{TODO: add table refs and refer to main text for method description}

\textbf{Comparison to literature (rev gUFv, yBMK, TZHc)}
We added a paragraph to \emph{Related Work} discussing budget-aware pruning and the relationship to our work. This paragraph can be found on page \bv{TODO: add page}. 

We also agree with reviewer TZHc that our work is influenced by the respective papers, albeit with important differences. We now make the similarities and differences more explicit, as indicated on pages \bv{TODO:add pages}.
\textbf{General importance of this work (rev  oGyB)}
We achieve accuracies that match or sometimes even surpass that of non-pruned networks and compete competitively among others. This is generally desirable in ML research. ML inference is a billion-\$ industry and users are most interested in more accurate methods. We further confirm the accuracy of our method in new analyses (see first two point above), achieving sometimes 15.96\% better accuracy \bv{TODO: add table ref}. As shown by these analyses, our method is also flexible as we have extended it to general budgeted pruning. Finally, our technique is easy to tune. e.g. CHIPNet adds 5 extra hyperparameters, while our work only introduces a single temperature hyperparameter which is easy to tune. In sum, we demonstrate a novel pruning technique, which is academically interesting, very accurate, easy to tune and can be flexibly applied to satisfy different resource constraints.

\textbf{Convergence (rev yBMK)}
We evaluate the wall-clock time by training ResNet-50 on a single A100 GPU for 300 iterations with a batch size of 64 by time.time() function. With/Without training a pruning mask, the average wall-clock time per iteration is 2.4413/2.4274 second/iteration. The training overhead increases by 0.5\% which is negligible. For the number of iterations to converge, it is dependent on mask dimensions and dataset and model architecture. In Fig.3(a) we show a small number of mask convergences. \bv{TODO: add fig ref}  

\textbf{Miscellaneous (rev TZHc)}
We have addressed the various additional comments on pages \bv{TODO:add pages}



%To compare with ChipNet, we use the default hyperparameters setting including learning rate, weight decay and  training epochs in the released code. 

\begin{table}
\centering
{
 \resizebox{1\linewidth}{!}{
\begin{tabular}{lccccccc} \toprule
  &  Temp. 1 &  Scale 1 & Temp. 2 & Scale 2 & Weightage 1 &  Weightage 2    \\ \midrule
CHIPNet:   & $\beta$  & $\beta_{inc}$      & $\gamma$ &  $\gamma_{inc}$  & $\alpha_1$ & $\alpha_2$   \\
Ours: &     $\varepsilon$      & -- &    --   & -- & -- &    --        \\ \bottomrule
\end{tabular}
} 
}% end color
\caption{ { Additional hyperparameters to tune for  ChipNet versus ours in learning a soft mask to satisfy the prescribed budgets. Here we use the channel budget  where the network is pruned to satisfy a global sparsity ratio, i.e., network wise sparsity. 
Our method only adds 1 additional hyperparameter to tune while ChipNet needs 6.
 } }
\label{tab:nrHyper}
\end{table}

\begin{table}[!t]
	\centering

\setlength{\tabcolsep}{1mm}{
	\renewcommand{\arraystretch}{1}
 \caption{MobileNetV2 on CIFAR-10/100: Channel budget i.e. global sparsity over network }
	\resizebox{1\linewidth}{!}{
		\begin{tabular}[c]{lc|ccc|ccccc}%{C{4cm}|C{2cm} C{2cm}}
			\toprule
			\multirow{2}{*}{Method} &  \multirow{2}{*}{Budget (\%)} & \multicolumn{3}{c|}{CIFAR-10 } &  \multicolumn{3}{c}{CIFAR-100}\\
			& & Acc. & Params.  & FLOPs & Acc. & Params.  & FLOPs   \\
			\midrule
   	Unpruned  & 100 &  93.70 & 100 & 100  & 72.80 & 100 & 100  
   \\
			\midrule

			ChipNet  &\multirow{2}{*}{80}& 92.23 & To-Calculate  &  & 72.25 &  &     \\
			Ours && 92.33 &  &  & 72.61 &  &     \\
   \midrule			
   ChipNet  &\multirow{2}{*}{60}& 92.24 &  &  & 70.62 &  &     \\
			Ours && 92.54 &  &  &   71.49 &  &     \\
   \midrule
   			ChipNet  &\multirow{2}{*}{40}& 91.83 &  &  & 66.61 &  &     \\
			Ours && 91.93 &  &  & 70.45 &  &     \\
   \midrule
   			ChipNet  &\multirow{2}{*}{20}& 90.41  &  &  & 52.96 &  &     \\
			Ours &&  91.49 &  &  &  68.90 &  &     \\
			\bottomrule
		\end{tabular}
	} 
 % \vspace{-0.1in}
}	
	\label{table:channelbudget}	
 % \vspace{-0.2in}
\end{table}



\begin{table}[!t]
	\centering
\caption{FLOPs budgets for WideResNet-26 on CIFAR-100}
\setlength{\tabcolsep}{1mm}{
	\renewcommand{\arraystretch}{1}
	\resizebox{0.6\linewidth}{!}{
		\begin{tabular}[c]{lc|cccccccc}%{C{4cm}|C{2cm} C{2cm}}
			\toprule
			\multirow{2}{*}{Method} &  \multirow{2}{*}{Budget (\%)} & \multicolumn{2}{c}{CIFAR-100 } \\
			& & Acc. & Params.    \\
			\midrule
   	Unpruned  & 100 &  80.21 & 100
   \\
			\midrule

			ChipNet  &\multirow{2}{*}{80}&  &        \\
			Ours &&   \\
   \midrule			
   ChipNet  &\multirow{2}{*}{60}&       \\
			Ours && &     \\
   \midrule
   			ChipNet  &\multirow{2}{*}{40}&   &     \\
			Ours &&  &      \\
   \midrule
   			ChipNet  &\multirow{2}{*}{20}&  77.15    &      \\
			Ours & & 78.17&   &     \\
			\bottomrule
		\end{tabular}
	} 
 % \vspace{-0.1in}
}	
	\label{table:FlopsBuget}	\vspace{-0.2in}
\end{table}




%\begin{itemize}
%    \item  TODO: Plot the learned pruning rate vs. epochs
%    \item 
%\end{itemize}

% \begin{itemize}
%     \item We are simplifying the model, why not lets simplify the algorithm itself! 
%     \item Related work to other budgets: not using logistic, not use STE.
% \end{itemize}

%We thank the reviewers for taking the time to review our manuscript and noting that we address an important problem (oGyB, gUFv, yBMK), with a novel and interesting pruning technique (oGyB, gUFv, yBMK), that achieves good results (oGyB, gUFv, TZHc), with a manuscript that is well organized, written, and motivated (oGyB, gUFv, yBMK). First, we provide a high-level summary of the changes that we've made to the draft to address your feedback, and conclude with an overview of our key contributions, and how they differ from previous work.

%Here is the summary of updates that we've made to the draft:

%\bv{TODO; just noticed we have only 1 page to respond, so this is too much text , we can prune once we have the figures}
%\bv{TODO: add HALP result to table 2? BUT uses per-network pruning}
%\bv{TODO: we should clearly mention that we cannot directly compare our ImageNet results to those of the budget-aware pruning methods because: 1. they use different objectives during training (e.g. latency, FLOPs), 2. they use network pruning (i.e. they can prune from any filter to satisfy their objective), while we apply layer-wise pruning with the exact same pruning rates as given by the CReg paper. So our search space is much more constraint (interestingly we still often do better). 3. their baseline model and hyperparameters are different, while we constrained our hyper-parameters to be equal to those in the CReg paper for fair comparison.}

%\textbf{Response to Reviewer 1}

%According to philosophy of science, science evolves through multiple phases. One of these phases, according to Thomas Kuhn, is \emph{normal science}. In this phase scientists build within a given paradigm increasingly better solutions for their problems. Deep learning currently experiences such a normal scienctific phase. Indeed, almost all published papers in machine learning build upon existing techniques in order to improve results on benchmark datasets. This paradigm has been incredibly successful, causing rapid progress on multiple tasks. As the reviewer acknowledges, our manuscript reveals a novel technique for pruning which achieves accuracies that match or sometimes even surpass the accuracy of non-pruned networks, and competes competitively among others. This is about as good as it gets in the current scientific phase of deep learning.

%As the reviewer rightfully points out, pruning is of much interest to industry players. It allows them to deploy models at much smaller compute, memory and energy costs. However, users are only happy with such optimized-performance solutions as long as their expected accuracy does not change too much. Indeed, when given the choice between two methods, all other things equal, users will always choose the more accurate method. Our method is currently the most accurate.

%During experimentation we noticed that our pruning method is not only very accurate on a range of networks and datasets, which we have further confirmed in additional analyses requested by other reviewers, we also noticed that our method is flexible, and relatively fast and easy to tune. Specifically, in the analyses below we show that we can extend our method to work with a fixed FLOP budget, on top of the fixed sparsity budget we already mentioned in the manuscript. We also show that, at least compared to some state-of-the-art methods, our pruning technique converges fast and has significantly less hyperparameters to tune.

%In sum, we show through multiple analyses that our pruning technique can be of substantial value to both science and industry.


%\textbf{Response to Reviewer 4}

%We agree with the reviewer that we were strongly inspired by ~\cite{xie2020differentiable} and ~\cite{xie2020fast}. First, like ~\cite{xie2020differentiable} our method builds upon well-established mathematical techniques from optimal transportation theory, such as minimizing the Wasserstein distance, entropic regularisation and Sinkhorn optimization. The paper ~\cite{xie2020differentiable} applies this methodology to the top-k operator for Image classification and beam search. In contrast, our work phrases neural network pruning as an optimal transport problem. Second, we build upon the work of ~\cite{xie2020fast} to make our pruning algorithm more efficient, requiring only 1 Sinkhorn iteration. Third, we extend the work of ~\cite{xie2020differentiable} and ~\cite{xie2020fast} by building upon the work of \cite{peyre2019computational, schmitzer2019stabilized} to automatically decay the temperature parameter $\varepsilon$. Finally, we apply our pruning method to a range of networks, using different datasets and pruning rates, and showing state-of-the-art results. Because of the inspiration we gathered from ~\cite{xie2020differentiable} and ~\cite{xie2020fast}, we cited those papers at the appropriate locations in the manuscript. However, we may not have credited these papers sufficiently so we have adjusted the manuscript to make this more explicit. We now write ... at p.x and write ... at p.y

%\bv{first version of extra paragraph to Related work section; TODO add refs}
%\noindent \textbf{Resource-aware channel pruning}
%Channel pruning was originally applied regardless of the particular benefits it would bring to inference on specific hardware platforms. However, recent works shows channel pruning in situations under which the resources of the compressed models must be restricted under certain budgets. Such budgeted pruning may target various resources such as volume budget (i.e. controlling the size of the activations held in memory), FLOPs budget (i.e. controlling the computational requirements of the model), parameter budget (i.e. controlling the storage of the model) and latency budget. Hence, budgeted pruning provides additional handles to optimize inference for particular applications on specific hardware. We show how our method can be extended to budgeted pruning using learnable pruning rates, which allows the model to automatically choose the distribution of pruning rates across layers.


==> revise_plan.tex <==
\clearpage
\section{--------------------Revise Plan--------------------}
\label{revise_plan}

\begin{itemize}
    \item  all minor things from reviewers \RVC{Done， Except for including automatic decaying schedule in Alg.1}
    \item extend related work: 1. budget-aware \RVC{Done}; 2. cite some other types pruning \RVC{Done}; 
    \item merge extra experiments: some (global sparsity on MobileNetv2, wall clock time, unstructured (as an additional experiment parag. ) to main paper \RVC{Done} and some (Flops or Latency budget) to appendix \RVC{Done, maybe revise later}
    \item Change the Alg.1 to 2 columns \RVC{Done}
    \item rewrite optimal transport related works: highlight the differences with ; \RVC{Done}
    \item remove unneeded appendix and revise figs like colors \RVC{Partially Done}
    \item extend intro to emphasize our contributions: 1. why learn mask is interesting; 2. why others like ChipNet not well; 3. why optimal transport(OT) and challenges of using OT; 4. How we solve and contributions \RVC{Done}
    \item polish abstract~\RVC{Done} and Bi-level optimization~\RVC{Done}
    \item rewrite discussion , limitations and future work \RVC{Partially Done}
    \item restructure the experiments, regroup some parts.~\yq{TODO}
    % \item Add one iteration optimization related works like Darts
    % \item share all checkpoints in anonymous link?

\end{itemize}
